Optimal by Design: Model-Driven Synthesis of Adaptation Strategies for Autonomous Systems

Many software systems have become too large and complex to be managed efficiently by human administrators, particularly when they operate in uncertain and dynamic environments and require frequent changes. Requirements-driven adaptation techniques have been proposed to endow systems with the necessary means to autonomously decide ways to satisfy their requirements. However, many current approaches rely on general-purpose languages, models and/or frameworks to design, develop and analyze autonomous systems. Unfortunately, these tools are not tailored towards the characteristics of adaptation problems in autonomous systems. In this paper, we present Optimal by Design (ObD ), a framework for model-based requirements-driven synthesis of optimal adaptation strategies for autonomous systems. ObD proposes a model (and a language) for the high-level description of the basic elements of self-adaptive systems, namely the system, capabilities, requirements and environment. Based on those elements, a Markov Decision Process (MDP) is constructed to compute the optimal strategy or the most rewarding system behaviour. Furthermore, this defines a reflex controller that can ensure timely responses to changes. One novel feature of the framework is that it benefits both from goal-oriented techniques, developed for requirement elicitation, refinement and analysis, and synthesis capabilities and extensive research around MDPs, their extensions and tools. Our preliminary evaluation results demonstrate the practicality and advantages of the framework.

==> Acknowledgment.tex <==
\section*{Acknowledgment}
	
This work was supported, in part, by Science Foundation Ireland grant 13/RC/2094 and ERC Advanced Grant 291652.
	

==> Submission Arxiv/Acknowledgment.tex <==
\section*{Acknowledgment}
	
This work was supported, in part, by Science Foundation Ireland grant 13/RC/2094 and ERC Advanced Grant 291652.
	

==> Submission Arxiv/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This paper introduces the \react framework for the model-based-require\-ments-driven synthesis of {\it reflex} controllers for autonomous systems. %In the framework, system models are separated from the underlying computational model, simplifying their design and maintenance by software engineers. More precisely, 
The framework introduces a model and a language to describe autonomous systems, their environment and requirements. The semantics of the model is defined in the form of an MDP, which can be solved producing optimal adaptation strategies (reflex controllers) for autonomous systems. In comparison with the general-purpose languages proposed by probabilistic model-checkers, \react solves two main limitations, namely the Markovian assumption and the implicit-event model. This enables the support of a comprehensive set of software requirements and permits the accurate modeling of the environment in which autonomous systems operate. 

%The semantics of the DSL is given in terms of MDP models. Solving these MDPs synthesizes {\it optimal reflex controllers} for the autonomous system. 

%Moreover, \react bridges the gap between goal modeling techniques and decision-theoretic planning (i.e. MDP), allowing to benefit from elicitation, refinement and analysis techniques of goal modeling frameworks and the computational machinery developed around MDPs and their many extensions and verification tools. %We have shown how several important types of $\text{`maintain'}$ and $\text{`achieve'}$ requirements are systematically supported in \react. Given requirements and a description of the autonomous system and its environment, we described how to construct an MDP to identify the optimal adaptation strategies or the most rewarding behavioral model of the autonomous system. We illustrated our approach through a running example. 

Future work consists of %adding support for probabilistic (or fuzzy) requirements~\cite{Grunske2008m,Calinescu2010,Baresi2010} and 
extending the framework to support %uncertainty in sensing (POMDP), continuous time~\cite{Calinescu2010,Iftikhar2014,Filieri2016}
 %(adversarial) multi-agent environments (Markov games~\cite{Camara2014a,Moreno2015,Camara2016}) and 
 online learning (reinforcement learning)~\cite{Tesauro2007}. The study of formal adaptation guarantees and assurances~\cite{Calinescu2017,Weyns2017a,Iftikhar2017a,Filieri2016}, and optimizing the performance of our framework~\cite{Pandey2016,Moreno2016} %and runtime adaptation~\cite{Iftikhar2014,Pandey2017,Su2017} 
 are other future planned extensions. %With respect to the current prototype, we plan to conduct a usability study and to integrate it into state-of-the-art (optimized) model checkers.
%\npaola{What about mentioning again here the usability study, the semantics extension needed for the assumptions which limit the applicability of the approach, and the integration with model optimized MC?}



==> Submission Arxiv/Context.tex <==
\section{Motivating Example}
\label{sec:running_example}
%Figure~\ref{fig:runningexample} shows the running example, inspired by one of the examples in~\cite{Skubch2013}. 
 %The figure shows the layout of a restaurant $FoodX$ which comprises three separate sections: (1) the kitchen, (2) the dining area and (3) the office. 
Our running example, inspired by one of the examples in~\cite{Skubch2013}, is the restaurant $FoodX$. Serving at $FoodX$ is $RoboX$, an autonomous mobile robot. The restaurant comprises three separate sections: (1) the kitchen, (2) the dining area and (3) the office. $RoboX$ is equipped with various sensors to monitor its environment and actuators to move around the restaurant and perform different tasks. 

Several challenges must be dealt with in order to develop a controller for $RoboX$. First, there are events that occur in the environment beyond $RoboX$'s control. For example, a client may request to order or a weak battery signal may be detected. There is also the uncertainty in action effects caused by imperfect actuators, e.g. moving to the kitchen from the dining room could sometimes fail, possibly due to the movement of customers in the restaurant. $RoboX$ may also have multiple (possibly conflicting) requirements: it may have to serve customers' food while it is still hot but also has to keep its batteries charged at all times. Thus, $RoboX$ should be able to prioritize the satisfaction of its requirements, taking into account the effects of their satisfaction over the long-term. It is also desirable that $RoboX$ acts proactively. For instance, waiting in the dining area should be preferred to staying in, for example, the kitchen if doing so would increase the likelihood of it getting orders from customers. %As a final requirement, it should be possible to support the runtime updating of the requirements guiding the behavior of $RoboX$ and, similarly, enabling the update of information about the system, environment and capabilities. 

Since the time and frequency of change in the environment cannot be controlled, enabling immediate and optimal responses to changes is highly desirable. In reactive approaches, {\it classical planning} (e.g., STRIPS~\cite{Fikes1971} and PDDL~\cite{mcdermott98pddl} planners) is often used to determine the best course of action after detection of change. This approach has important limitations. For example, imagine a situation where, while $RoboX$ is moving to serve a customer in the dining room, a weak battery signal is detected. In this case, $RoboX$ can either halt the execution of the current plan until a new plan is computed or continue pursuing serving the customer, having no guarantees that this plan is still the optimal course of action. If the frequency of changes in the environment is high, then the autonomous system may get permanently stuck computing new plans, or be always following sub-optimal plans. %Generally, adaptation is performed using a  Monitor-Analyze-Planning-Execute (MAPE) paradigm~\cite{Kephart2003} where {\it classical planning} (i.e., STRIPS~\cite{Fikes1971} and PDDL~\cite{mcdermott98pddl}) is traditionally used to determine the best course of action when a change is detected. This reactive paradigm is inadequate, unless computation of plans is instantaneous. For example, imagine if while $RoboX$ is moving to serve a customer in the dining room, a weak battery signal is detected. In this case, it is possible to halt execution of the current plan until a new plan is computed or continue plan execution with no optimality guarantees. If the frequency of changes detected is high, then this situation is worsened as the autonomous system would be either permanently stuck computing new plans, or pursuing plans with no guarantees of their optimality. 

This example highlights the five requirements for the software to control $RoboX$ which we explore in this paper: %Those requirements are:
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth,height=0.5\linewidth]{RunningExample_2}
%	\caption[Restaurant Layout]{$FoodX$ Restaurant Layout}
%	\label{fig:runningexample}
%\end{figure}

%\subsection{Requirements for Controlling $RoboX$}
%\label{sec:discussion_of_motivating_example}

\begin{enumerate}
	\item Handling of uncertainty in event occurrences and effects;
	\item Proactive and long-term behavior optimization to consider the possible evolution of the system when determining the best course of action;
	\item Fast and optimal response to changes to ensure their ability to operate in highly dynamic environments;
	\item Support of requirements trade-offs and prioritisation;
	\item Support of requirements-driven adaptation to raise the level of abstraction of system design.
\end{enumerate}

%\paragraph{Support of requirements trade-offs} Requirements specify the system's objectives. However, those objectives often conflict. For example, it may be required that $RoboX$ charges its batteries and, at the same time, brings food to a customer's table. In this case, it may not be possible to satisfy both these requirements. A disciplined trade-off of requirements according to their relative importance is therefore needed.
\comments{
\paragraph{{\bf C$_1$} - Handling of uncertainty} in occurrence of events and action effectsMany sources of uncertainty have been identified in self-adaptive systems~\cite{Esfahani2013}. In our running example, two main sources of uncertainties can be identified. Firstly, there are exogenous events that occur in the environment beyond $RoboX$'s control. %For example, a client might request to order at anytime or a weak battery signal may be detected. Secondly, there is the uncertainty in action effects caused by imperfect actuators. For example, moving to the kitchen from the dining room could sometimes fail due to the movement of customers in the restaurant. 


\paragraph{Proactive and long-term behavior optimization} As opposed to reactive adaptation where the system only reacts when a requirement is violated, proactive behavior considers the possible evolution of the system to determine the best course of action. %For example, it could be better to not serve a customer and immediately charge $RoboX$'s if there is a high likelihood that a low battery signal be detected; or waiting in the dining area may be preferred to waiting in the kitchen if this would maximize the satisfaction of requirements, e.g., getting orders from customers.  

\paragraph{Fast and optimal response to change}\paola{this is a fuzzy quantity} In an uncontrollable environment, the time and frequency of changes cannot be controlled. Guaranteeing immediate and optimal responses to changes is therefore highly desirable. Traditionally, adaptation is performed using a  Monitor Analyze Planning Execute (MAPE) paradigm where classical planning (see for example STRIPS~\cite{Fikes1971} PDDL~\cite{mcdermott98pddl}) is used to determine the best course of action when a change is detected. This reactive paradigm is inadequate, unless the computation of plans is instantaneous. For example, imagine if while $RoboX$ is moving to serve a customer in the dining room, a weak battery signal is detected. In this case, it is possible to halt the execution of the plan until a new plan is computed or resume the execution of the current plan with no guarantees of its optimality. If the frequency of changes detected in the environment is high, then this situation is worsened as the autonomous system would be permanently stuck in a state where it is computing plans without acting, or it would be indefinitely pursuing plans with no guarantees of their optimality. The computation of an {\it optimal strategy} provides a solution to this problem. An optimal strategy identifies the best adaptation action that should be taken in every possible evolution of the system. Thus, it enables an almost instantaneous response to every possible change since optimal responses are precomputed, eliminating the need to re-plan after every change\paola{I don’t think it is clear how this guarantee instantaneous respone }. In other words, the computation of a strategy defines a {\it reflex controller} for the autonomous system that enables it to optimally and instantaneously react to every possible future change.

 \paragraph{Support of a model-based-requirements-driven adaptation}\paola{Why the kind of the adaptation is part of the requirement? Shouldn’t it be part of the solution?} Requirements are prescriptive statements of intent to be satisfied by cooperation of the agents forming the system~\cite{Lamsweerde2009}. They say what the system will do and not how it will do it~\cite{Zave1997}.\paola{This shouldn’t be part of this but outside} In complex and nondeterministic environments, it is very difficult to anticipate and explicitly prescribe the system's ideal behavior in every situation. A model-based approach where requirements are used to drive system adaptation provides several advantages. First, it raises the level of abstraction at which the system should be designed and analyzed and allows to benefit from works on requirements elicitation, refinements and analysis produced over the years in Requirements Engineering (RE)~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017}\paola{why?}. Second, it relieves the software engineer from the heavy task of prescribing the strategies that are needed to adapt the system when changes occur.
}


\comments{
\subsection{Summary of Challenges}
\label{sec:challenges}

The software of an autonomous robot such as $RoboX$ must satisfy various requirements. First, it must 

enable it to satisfy its various goals and requirements. For example, after getting an order, $RoboX$ must also ensure that the order is given to the kitchen and that subsequently food is delivered to the table. It may also need to charge its batteries after a low battery signal is detected. Obviously, these requirements may conflict. Therefore, $RoboX$ must be endowed with the intelligence necessary to optimize the satisfaction of its various (possibly conflicting) requirements according to the present situation.

There are several ways to define a controller for $RoboX$. One possibility is to predefine all possible situations and specify how the robot should behave in each. This solution is impractical as there are potentially millions of situations which would need to be covered. To rely on the Monitor Analyze Planning Execute (MAPE-K) paradigm could be a better alternative: the robot monitors the environment, plans its best course of action accordingly and then executes the plan. However, the use of planning has some shortcomings. For example, it is not suitable for handling of uncertainty during plan execution. For example, if while the robot is executing some plan, a customer places an order, should the current plan be abandoned or resumed? If the robot decides to resume the plan, then it might be pursuing a sub-ideal plan. On the other hand, if it decides to recompute its plan, then frequent occurrences of events in its environment may prevent it from executing any plan altogether. Furthermore, actuators of $RoboX$ may not be perfect and may not necessary always produce their desired effects. For example, it could be the case that moving to the kitchen from the dining room may sometimes fail, due to the movement of customers in the restaurant. 

Besides dealing with uncertainty, there is the need to deal with multiple (possibly conflicting) requirements. For example, this may happen if $RoboX$ should charge its batteries and bring food to a customer's table while it is still hot. There is therefore a need to support disciplined trade-off of requirements that is based on reasoning about the importance of requirement satisfaction. In order to do so, there should be a reward or utility function which specifies the expected return or payoff for requirements satisfaction and $RoboX$ should choose its actions such that they maximize  this reward or utility function. 

Thus, to deal with the aforementioned challenges, the software of $RoboX$ should aim at the {\it optimal} satisfaction of its {\it requirements}~\cite{Zave1997,Lamsweerde2009} given a description consisting of the system and its environment. Notice that requirements say what the system will do and not how it will do it~\cite{Zave1997}. Thus, they enable to raise the level of abstraction of system specifications and reduce considerably the size of system specifications that have to be provided. 

To identify the optimal behavior of the system based on a high-level description of the system, its environment and its requirements, we construct a Markov Decision Process (MDP). By solving this MDP, we can compute an {\it optimal} strategy that identifies the action that should be taken in every possible situation in order to best satisfy the requirements of $ROboX$. 

One important benefit of this approach is that relying on requirements for the generation of strategies makes possible to benefit from works on requirements elicitation, refinements and analysis produced over the years in Requirements Engineering (RE)~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017}. It also enables to benefit from the powerful computational machinery that comes with Markov Decision Models and its extensions and tools.


We summarize the following main challenges for the software that controls $RoboX$:
\begin{itemize}
	\item High-level specification of goals/requirements: it is impractical to predict every possible situation and predefine a good response to it. It would therefore be much more convenient to support the specification of high-level goals for the robot and provide it with the means necessary to determine its best course of action according to the current context or situation;
 
	\item Handling uncertainty in the environment: $RoboX$ must be able to react optimally, and instantly if possible, even when exogenous events beyond its control occur in its environment;
	
	 
	\item Handling of non-determinism: actuators of $RoboX$ may not always produce the desired outcomes. Similarly, events may not have deterministic effects. Therefore, it is highly desirable that this kind of uncertainty be considered when $RoboX$ decides of its best course of action.
\end{itemize}

%The computation of an {\it optimal strategy} provides a solution to this problem. An optimal strategy identifies the best adaptation action that should be taken in every possible evolution of the system. Thus, it enables an almost instantaneous response to every possible change since optimal responses are precomputed, eliminating the need to re-plan after every change\paola{I don’t think it is clear how this guarantee instantaneous respone }. In other words, the computation of a strategy defines a {\it reflex controller} for the autonomous system that enables it to optimally and instantaneously react to every possible future change.


%$RoboX$ needs to make best use of its capabilities to serve customers of $FoodX$. %In the dining area, there are several tables where customers can sit and order food. In the office, there is a battery charging station. 
}




==> Submission Arxiv/Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
%\react supports the computation of optimal strategies based on requirements in a variety of situations. 
%The theoretical complexity of the computation of MDP strategies is well-known~\cite{Baier:2008:PMC:1373322,Mausam2012}.%\footnote{The current implementation uses the MDPToolBox package~\cite{MDPToolbox2017} for solving MDPs. An integration of \react into PRISM is planned.}. 
%To evaluate \react, there are three different aspects to consider:
%\begin{itemize}
%\item the advantages of using \react to identify optimal adaptation strategies for autonomous systems;
%\item the scalability of the approach;
%\item the usability of \react as modeling language and framework.
%\end{itemize}
In this section, we first present an empirical evaluation of the framework by comparing the use of an \react controller to control $RoboX$ in a simulated software environment of the restaurant $FoodX$ to a generic Monitor Analyze Plan Execute (MAPE) controller (Section~\ref{sec:empirical_evaluation}). The MAPE controller relies on a Planning Domain Description Language (PDDL) planner, similarly to state-of-the-art robotic systems such as ROS~\cite{rosplan}. 
Then, we present a qualitative comparison of \react with state-of-the-art probabilistic model-checkers, PAT~\cite{SunLDP09}, PRISM~\cite{Kwiatkowska2011} and STORM~\cite{Dehnert2017} which have been used in several other previous works~\cite{Camara2014a,Camara2015,Moreno2015,Camara2016} to solve adaptation problems (Section~\ref{sec:comparison_probabilistic_model_checkers}). Finally, we describe the current prototype tool implementation and conduct a performance evaluation (Section~\ref{sec:preliminaryeval}). 



%are better captured in \react than in turn-based PRISM-games. In particular, in turn-based Markov games, at each turn, one player selects one action to execute, which means that, if the environment is modeled as an agent then at most one exogenous event may occur after each action of the agent. The modeling of the environment in \react is therefore more natural since multiple events may occur with each action of the agent, each according to their occurrence probability. 

%In this section, we will focus on the first two aspects by presenting an analysis of the benefits of \react (Section~\ref{sec:action_costs}) and a preliminary evaluation of the performance of a prototype implementation (Section~\ref{sec:preliminaryeval}). The usability study to assess the user-friendliness of the framework is planned as a future work. 
%Since one of the main contribution of the proposed approach is a language in which system and requirements are kept separated, in order to verify the usability of the approach, we are planning to conduct usability testing and a controlled experiment.
%
%\comments{
%\subsection{Achieve and Maintain Requirements}
%\label{sec:classical_planning}
%Consider the following domain description: 
%\begin{align*}
%	&\textbf{Action } move\_to\_kitchen\\
%	& \hspace{1cm} \textbf{ if } location=hallway \textbf{ effects } \langle location=kitchen\rangle\\
%	&\textbf{Action } move\_to\_hallway\\
%	& \hspace{1cm} \textbf{ if } location=dining\_room \,|\, location=kitchen \,|\, \\
%	& \hspace{1cm} location=office \textbf{ effects } \langle location=hallway\rangle\\
%	&\textbf{Action } move\_to\_office\\
%	& \hspace{1cm} \textbf{ if } location=hallway \\
%	& \hspace{1cm}\textbf{ effects } \langle location=office\rangle\\
%	&\textbf{Action } move\_to\_dining\_room\\
%	& \hspace{1cm} \textbf{ if } location=hallway \,|\, location=table_i \\
%	& \hspace{1cm}\textbf{ effects } \langle location=dining\_room \rangle \hspace{1cm} (\forall 1\leq i \leq 4)\\
%	&\textbf{Action } move\_to\_table_i\\
%	& \hspace{1cm} \textbf{ if } location=hallway \,|\, location=table_i\\
%	& \hspace{1cm} \textbf{ effects } \langle location=table_i \rangle \hspace{1cm} (\forall 1\leq i \leq 4)\\
%	&\textbf{ReqID } req_1 \textbf{ achieve (maintain) } location=office 
%\end{align*}
%\noindent In the previous domain description, all actions are deterministic and there is only one (unconditional) requirement to achieve (maintain) $location=office$. The computed strategy determines the optimal action, in every state, which execution maximizes the expected reward, i.e. satisfaction of requirements. Fig~\ref{fig:evaluationexample1} shows the computed strategy for a selected set of states: namely when $RoboX$ is at table 1 ($s_0$), in the dining room ($s_1$), in the hallway ($s_2$) and in the office ($s_3$). When the requirement is an unconditional achieve, the optimal strategy for the agent is to aim at satisfying the requirement {\it as many times as} possible by repeatedly moving into and out from the office. On the other hand, when the requirement is a maintain requirement, the agent tries to satisfy the requirement {\it as long as} possible by remaining in the office. 
%
%
%This example illustrates the difference between classical planning and the use of MDP: in the former, a finite sequence of action is identified to reach a desired goal whereas in the latter the computed strategy determines the action to execute at each possible state that would maximize the total expected rewards. Thus, the latter computes an optimal behavior as opposed to a simple course of action. %It is thus more suitable for determining the {\it operational} system which does not stop when some end goal is achieved but have (several possibly conflicting) requirements to satisfy.
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{EvaluationExample1}
%	\caption{Unconditional (a) Achieve and (b) Maintain Requirements}
%	\label{fig:evaluationexample1}
%\end{figure}
%}

\subsection{Empirical Evaluation}
\label{sec:empirical_evaluation}
Figure~\ref{fig:simulation} depicts our simulation environment. It consists of a system state, an agent and an environment. The simulation runs in discrete time steps. At each step, the agent has to choose, based on the current system state, one action to execute from actions whose preconditions are satisfied in the state. On the other hand, some events are selected for execution, according to their occurrence probability, if their preconditions are true. After each time step, the state is updated by applying the effects of the chosen action and events in the current state. Effects of both actions and events are applied probabilistically according to the probabilities specified in their action/event descriptions, i.e. their execution can lead to different states. Experiments are run for one hundred thousands steps.

To select the agent's actions, two controllers were implemented: an \react controller and a generic MAPE controller. The design rational of the experiment aims at comparing a \react controller and generic MAPE controllers with respect to: types of supported requirements, enforcement model, response time, quality of decision-making and problem representation.
%\end{itemize}

\paragraph*{Experiment Description} The experiment ran on a MacBook pro with a 2.2GHz Intel Core i7 and 16 GB of DDR3 RAM. At each time step, the agent queries the state (the (M)onitoring activity). The agent determines its action to execute by interacting with its controller. The controller, given the current state, determines the next action of the agent. %Two controllers were used: an \react controller and a generic MAPE controller. 
The \react controller is implemented in Java and uses the computed \react strategies to determine the optimal action that the agent should take at each state. The MAPE controller is also implemented in Java. It consists of three components: 1) an analysis component that determines whether planning is needed, 2) PDDL4J, an open source Java library for Automated Planning based on PDDL~\cite{PDDL4J}, to compute plans and 3) a plan enforcer which returns one action at each step to the agent. Below is a comparison of the two controllers.

\paragraph*{Supported requirements} \react supports the types of requirements presented in Section~\ref{sec:modeling_requirements}. The MAPE controller, since it relies on a PDDL planer, can naturally encode unconditional and conditional achieve requirements, i.e. $\langle UA, CA\rangle$. The other types of requirements cannot be easily encoded in the form of PDDL planning problems. %Other requirements, i.e. $\langle DEA,DFA,$$DEM,DFM,PM,$$PDEM,PDFM,$$RPM,$ $RPDEM,RPDEM\rangle$ are not supported. %For example, it is not possible to state that RoboX should charge its battery for a certain duration and that this condition should be achieved within a certain deadline. Similarly, it is not possible to specify requirements cancellation condition, i.e. state that a plan should not longer be pursued if a certain condition becomes true while the execution of the plan.


\paragraph*{Enforcement model} The \react controller enforces MDP strategies. It has a simple enforcement model: it consults the computed strategy and determines the optimal action that corresponds to the current state at each time step. The MAPE controller enforces requirements as follows: if the activation condition of a conditional requirement is true in the state then a planning problem (Pb) is formulated to satisfy the requirement's condition. When multiple requirements must be satisfied, then the goal state of the planning problem corresponds to the disjunction of their (satisfaction) conditions, i.e. one requirement should be satisfied. If a plan (P) is found by the PDDL planner, the plan enforcer module selects one action of P to return to the agent at each time step. A plan is pursued until its end, i.e. no re-planning is performed until the plan's last action is executed unless a plan execution fails. A plan fails if one of its actions cannot be executed because its preconditions are not satisfied in the current state. This situation may occur due to nondeterministic action effects or event occurrences\footnote{Another situation where re-planning would be required is cancellation of requirements. This situation is not considered in this experiment for simplicity.}. 


\begin{figure*}[!htb]
%\resizebox{\textwidth}{0.15\textwidth}{
	\minipage{0.32\textwidth}
		\includegraphics[scale=0.3]{Simulation}
		\caption{Experiment Description}\label{fig:simulation}
	\endminipage\hfill
	\minipage{0.32\textwidth}
%		\resizebox{\textwidth}{\textwidth}{
		\begin{tikzpicture}[scale=0.6]
	\begin{axis}[ylabel=decision-making time per time step,xlabel=nb of planning goals]
	\addplot coordinates {
		(0,0)
		(4,261)
		(8,294)
		(12,288)
	};
	\addplot coordinates {
		(0,0)
		(4,284)
		(8,378)
		(12,370)
	};
	\addplot coordinates {
		(0,0)
		(4,348)
		(8,488)
		(12,463)
	};
	\addplot coordinates {
		(0,0)
		(4,409)
		(8,586)
		(12,556)
	};
	\addplot coordinates {
		(0,0)
		(4,514)
		(8,689)
		(12,639)
	};
	\addplot coordinates {
		(0,0)
		(4,593)
		(8,719)
		(12,724)
	};
	
	\addplot coordinates {
		(0,0)
		(4,0.2)
		(8,0.3)
		(12,0.25)
	};
	
	\addlegendentry{M-100\%}
	\addlegendentry{M-90\%}
	\addlegendentry{M-80\%}
	\addlegendentry{M-70\%}
	\addlegendentry{M-60\%}	
	\addlegendentry{M-50\%}
	\addlegendentry{A-all}
	\end{axis}
	\end{tikzpicture}

\caption{Decision-making time per time step}
\label{lab:fig_response}
	\endminipage\hfill
	\minipage{0.32\textwidth}%
%		\resizebox{\textwidth}{\textwidth}{
	\begin{tikzpicture}[scale=0.6]
\begin{axis}[ylabel=nb of satisfied goals per time step,xlabel=nb of planning goals]
\addplot coordinates {
	(0,0)
	(4,0.2)
	(8,0.228)
	(12,0.24)
};
\addplot coordinates {
	(0,0)
	(4,0.152)
	(8,0.208)
	(12,0.216)
};
\addplot coordinates {
	(0,0)
	(4,0.14)
	(8,0.188)
	(12,0.192)
};
\addplot coordinates {
	(0,0)
	(4,0.128)
	(8,0.164)
	(12,0.168)
};
\addplot coordinates {
	(0,0)
	(4,0.116)
	(8,0.144)
	(12,0.124)
};
%		\addplot coordinates {
%			(0,0)
%			(4,26)
%			(8,30)
%			(12,25)
%		};

\addlegendentry{M-100\%}
\addlegendentry{M-90\%}
\addlegendentry{M-80\%}
\addlegendentry{M-70\%}
\addlegendentry{M-60\%}	
%\addlegendentry{M-50\%}
\addplot coordinates {
	(0,0)
	(4,0.2)
	(8,0.264)
	
};
\addplot coordinates {
	(0,0)
	(4,0.188)
	(8,0.244)
	
	
};
\addplot coordinates {
	(0,0)
	(4,0.176)
	(8,0.224)
	
};
\addplot coordinates {
	(0,0)
	(4,0.16)
	(8,0.204)
	
};
\addplot coordinates {
	(0,0)
	(4,0.144)
	(8,0.18)
	
};
%		\addplot coordinates {
%			(0,0)
%			(4,32)
%			(8,39)
%			
%		};

\addlegendentry{A-100\%}
\addlegendentry{A-90\%}
\addlegendentry{A-80\%}
\addlegendentry{A-70\%}
\addlegendentry{A-60\%}	
%\addlegendentry{A-50\%}
\end{axis}
\end{tikzpicture}
%}
\caption{Goal satisfaction per time step} \label{fig:rewards_mape_react}
	\endminipage
%}
\end{figure*}

%\begin{figure}
%	\begin{center}
%		\begin{tikzpicture}
%		\begin{axis}[ylabel=decision-making time per time step,xlabel=nb of planning goals]
%		\addplot coordinates {
%			(0,0)
%			(4,261)
%			(8,294)
%			(12,288)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,284)
%			(8,378)
%			(12,370)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,348)
%			(8,488)
%			(12,463)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,409)
%			(8,586)
%			(12,556)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,514)
%			(8,689)
%			(12,639)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,593)
%			(8,719)
%			(12,724)
%		};
%		
%		\addplot coordinates {
%			(0,0)
%			(4,0.2)
%			(8,0.3)
%			(12,0.25)
%		};
%		
%		\addlegendentry{M-100\%}
%		\addlegendentry{M-90\%}
%		\addlegendentry{M-80\%}
%		\addlegendentry{M-70\%}
%		\addlegendentry{M-60\%}	
%		\addlegendentry{M-50\%}
%		\addlegendentry{A-all}
%		\end{axis}
%		\end{tikzpicture}
%	\end{center}
%	\caption{Average decision-making time per time step: MAPE vs. \react}
%	\label{lab:fig_response}
%\end{figure}
\paragraph*{Response time} Figure~\ref{lab:fig_response} shows the average time of decision making, i.e. the total decision-making time divided by the total number of steps of the experiment. Several domain descriptions differing in their total number of planning goals/requirements and action success rate\footnote{Action success means that the action produced its (expected) effect, i.e. the effect that is most likely to occur.} (100\%-50\%) are considered. The decision time of an \react controller is constant and almost instantaneous ($\sim$200ns) as it consists of a simple lookup in the policy (which is stored in the form of an array of Integers) of the optimal action that corresponds to the current state. On the other hand, the analysis and planning activities of the MAPE controller introduce a significant overhead when compared to the \react controller. The average decision-making time of MAPE controllers also increases with action non-determinism as re-planning is required more frequently due to more frequent plan failures.  

%\begin{figure}
%	\begin{center}
%		\begin{tikzpicture}
%		\begin{axis}[ylabel=nb of satisfied goals per time step,xlabel=nb of planning goals]
%		\addplot coordinates {
%			(0,0)
%			(4,0.2)
%			(8,0.228)
%			(12,0.24)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.152)
%			(8,0.208)
%			(12,0.216)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.14)
%			(8,0.188)
%			(12,0.192)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.128)
%			(8,0.164)
%			(12,0.168)
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.116)
%			(8,0.144)
%			(12,0.124)
%		};
%%		\addplot coordinates {
%%			(0,0)
%%			(4,26)
%%			(8,30)
%%			(12,25)
%%		};
%		
%		\addlegendentry{M-100\%}
%		\addlegendentry{M-90\%}
%		\addlegendentry{M-80\%}
%		\addlegendentry{M-70\%}
%		\addlegendentry{M-60\%}	
%		%\addlegendentry{M-50\%}
%		\addplot coordinates {
%			(0,0)
%			(4,0.2)
%			(8,0.264)
%			
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.188)
%			(8,0.244)
%
%			
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.176)
%			(8,0.224)
%			
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.16)
%			(8,0.204)
%			
%		};
%		\addplot coordinates {
%			(0,0)
%			(4,0.144)
%			(8,0.18)
%			
%		};
%%		\addplot coordinates {
%%			(0,0)
%%			(4,32)
%%			(8,39)
%%			
%%		};
%		
%		\addlegendentry{A-100\%}
%		\addlegendentry{A-90\%}
%		\addlegendentry{A-80\%}
%		\addlegendentry{A-70\%}
%		\addlegendentry{A-60\%}	
%		%\addlegendentry{A-50\%}
%		\end{axis}
%		\end{tikzpicture}
%	\end{center}
%	\caption{Average goal satisfaction per time step of MAPE (M) and \react (A) controllers}
%		\label{fig:rewards_mape_react}
%\end{figure}

\paragraph*{Quality of decision-making} Figure~\ref{fig:rewards_mape_react} shows the number of satisfied goals per time step for MAPE and \react controllers. It demonstrates that the \react controllers consistently outperform MAPE controllers for the same domain problems. This is due, on one hand, to their ability to include probabilities of event occurrences into their computation of optimal strategies. For instance, imagine that $RoboX$ has to pass the order of a table to the kitchen but that it estimates that there is a high-likelihood that another table orders. In this case, the \react controller may delay moving to the kitchen to pass the order and wait until the other table orders first before passing the two orders to the kitchen together. MAPE controllers are incapable of incorporating such intelligence in their decision-making. Another reason explaining this result is that MAPE controllers, once a plan is computed, commit to it unless the plan fails to avoid getting stuck in re-planning without acting, which could happen if the frequency of change in the environment is high. This makes it impossible to guarantee the optimality of plans throughout their execution. On the other hand, \react strategies are guaranteed to always select the optimal action at each state.

\paragraph*{Representation} An important difference is the goal/requirement representation. In MAPE, planning goals have to be satisfiable using solely the actions that are available to the agent. For example, consider a goal to achieve that a table pays as many times as possible. The satisfaction of this goal requires interactions with the environment as described in Figure~\ref{fig:tablelts}. This requirement cannot therefore be expressed as a single planning goal but has to be decomposed into a set of planning goals, each of which has to be satisfiable by the actions available to the agent. On the other hand, thanks to the folding of events into actions, such requirements can be expressed directly in \reactt. Consequently, expression of requirements in \react can be much more succinct and enable system designers to focus of what should be satisfied rather than how they should be satisfied. In the running example, it was possible to represent four MAPE planning goals in the form of a single \react requirement.  



\subsection{Qualitative Comparison of \react with State-of-the-Art Probabilistic Model-checkers}
\label{sec:comparison_probabilistic_model_checkers}
 State-of-the-art probabilistic model-checkers PAT~\cite{SunLDP09}, PRISM~\cite{Kwiatkowska2011} and STORM~\cite{Dehnert2017} support the description of various models using a variety of languages. In this work, we focus on MDP models because they support, as opposed to other models such as for example Discrete-Time Markov Chains, the synthesis of optimal strategies. With respect to the general-purpose languages proposed by probabilistic model-checkers, our model and language support exogenous events and various typical software requirements (Section~\ref{sec:modeling_requirements}), elements that cannot be modeled or expressed using the general-purpose MDP languages of PAT, PRISM or Storm. An extension of PRISM, namely PRISM-games, supports modeling of turn-based multi-player stochastic games. This enables the modeling of the environment as a separate player whose actions represent exogenous events. With respect to modeling of autonomous systems and their requirements, PRISM-games has two main limitations. First, similarly to PRISM, rewards have to be Markovain which means that there is no way to encode typical software requirements~\cite{Lamsweerde2009} such as those presented in Section~\ref{sec:modeling_requirements} using the provided (Markovian) reward structures. Furthermore, modeling of interactions between the agent and its environment in \react where multiple events occur with each action of the decision maker is more realistic and natural than, in turn-based PRISM-games, where the environment may only be represented in the form of a separate player who selects at most one event to execute after each action of the decision maker.

\comments{
\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{Simulation}
	\caption{Simulation Description}
	\label{fig:simulation}
\end{figure}


\subsection{The benefits of \react}
\label{sec:action_costs}

%\paragrph{Trading off Rewards and Action Costs}
%In the absence of action costs, the satisfaction of every requirement brings some benefit to the agent. However, when actions are associated with a cost, the satisfaction of requirements is traded-off against the total cost of action executions needed to satisfy them. For example, consider the following  domain description:
%\begin{align*}
%	&\textbf{Action } move\_to\_kitchen \textbf{ if } location=hallway \\
%	& \hspace{0.5cm} \textbf{ effects } \langle location=kitchen\rangle\\
%	& \textbf{Action } move\_to\_hallway \textbf{ if } location=dining\_room \,|\,\\
%	& \hspace{0.5cm}  location=kitchen \,|\, location=office  \\
%	& \hspace{0.5cm} \textbf{ effects } \langle location=hallway\rangle\textbf{ cost } 30\\
%	& \textbf{Action } move\_to\_office\textbf{ if } location=hallway  \\
%	& \hspace{0.5cm} \textbf{ effects } \langle location=office\rangle \textbf{ cost } 80\\
%	&\textbf{Action } move\_to\_dining\_room\\
%	& \hspace{0.5cm} \textbf{ if } location=hallway \,|\, location=table_i \\
%	& \hspace{0.5cm}\textbf{ effects } \langle location=dining\_room \rangle\\
%	&\textbf{ReqID } req_1 \textbf{ achieve (maintain) } location=office \textbf{ reward } 100
%\end{align*}
%\noindent In this case, the actions {\it move\_to\_hallway} and {\it move\_to\_office} have a cost of 30 and 80 respectively. The strategy for the $\text{`achieve'}$ requirement determines that the agent should move into the office only it is already in the hallway (see Fig~\ref{fig:action_cost_example}(b)). At every other location, the optimal action is the {\it noop} action since the total cost of moving to the hallway and then into the office exceeds the expected reward from satisfying the requirement. On the other hand, the strategy computed for the maintain requirement moves the agent into the office as shown in Fig~\ref{fig:action_cost_example}(a). This is because a reward is obtained at every time step the {\it maintain} requirement is satisfied, thus the total expected reward is bigger than the total cost of action executions. 
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{ActionCostExample}
%	\caption{Trade-offs between Action Costs and Requirements}
%	\label{fig:action_cost_example}
%\end{figure}
As discussed in Section~\ref{sec:running_example}, many of the difficulties of adaptation in autonomous systems stem from uncertainties in the system, its environment and conflicts that arise when multiple requirements have to be satisfied at the same time. This section focuses on showing how \react deals with those challenges through use case examples.% These issues are conveniently resolved in \react as demonstrated in this section. 


\paragraph*{Dealing with Uncertainty}

\react allows the modeling of two sources of uncertainty: (1) action/event effects, and (2) occurrence of exogenous events. 

\textit{Effects} For example, imagine that $RoboX$ has to move to the office, which can be accessed in two ways: 1) directly from $table_2$ through a small door but that due to the size of the door, $RoboX$ succeeds to pass through the door only \textit{Pb}\% of the time, 2) indirectly by moving to the dining room, then to the hallway and finally into the office. This can be modeled by adding an action {\it move\_from\_table\_2} and a requirement $req\_1$ to the domain description:
\begin{align*}
	&\textbf{ReqID } req_1 \textbf{ achieve } location=inOffice\\ 
		&\textbf{Action } move\_from\_table_2 \textbf{ if } location=atTable_2\\
	& \hspace{1cm}  \textbf{ effects } \langle location=inOffice  \textbf{ prob } Pb\rangle 
\end{align*}

\noindent %Consequently, $RoboX$ can move to the office when it is at table 2 by either: (1) moving to the dining room then into the hallway then into the office or, (2) moving directly to the office. 
The computation of an optimal strategy determines that for every $Pb < .33$, $RoboX$'s optimal course of action is to take the longer route since it would be expected that fewer steps would be needed to move into the office. For every $Pb>=.33$, moving directly into the office from $table_2$ is the optimal action.  

\textit{Exogenous Events} In the running example, several exogenous events may occur: a customer may arrive, they may request to place an order, they may order, pay or leave. Those exogenous events may have preconditions. For example, it is possible that when new customers arrive, they occupy the first available table. For example, customers sit at $table_1$ if it is available, i.e., $table_1=empty$. Otherwise, they move to the next available table. This may be expressed as follows:

\begin{align*}
	&\textbf{Event } customer\_arrives\\
	& \hspace{0.5cm} \textbf{ if } table_1=empty \textbf{ occur prob } 0.1 \textbf{ effects } \langle table_1=occupied  \rangle \\
	& \hspace{0.5cm} \textbf{ if } !table_1=empty \,\&\, table2=empty \textbf{ occur prob } 0.1 \\
	& \hspace{0.7cm} \textbf{ effects } \langle table_2=occupied  \rangle \\
	& \hspace{0.5cm}...\\
	%&\textbf{Event } customer\_requests_i\\
	%& \hspace{1cm} \textbf{ if } table_i=occupied \,\&\, location=dining\_room \textbf{ occur prob } 0.2\\
	%&\hspace{1cm}\textbf{ effects } \langle table_i=requested \rangle\\
	&\textbf{Event } customer\_orders_i \textbf{ if } table_i=requested \,\&\, location=\\
	& \hspace{0.5cm}  atTable_i \textbf{ occur prob } 0.8 \textbf{ effects } \langle table_i=received \textbf{ prob } 0.8 \rangle\\
	&\textbf{Event } customer\_pays_i \textbf{ if } table_i=delivered \\
	& \hspace{0.5cm} \textbf{ occur prob } 0.2\textbf{ effects } \langle table_i=paid  \rangle \\
%	&\textbf{Event } customer\_leaves_i\\
%	& \hspace{1cm} \textbf{ if } table_i=paid \textbf{ occur prob } 0.3\textbf{ effects } \langle table_i=occupied  \rangle \\
	&\textbf{Event } order\_ready_i \textbf{ if } table_i=in\_preparation \\
	& \hspace{0.5cm} \textbf{ occur prob } 0.2\textbf{ effects } \langle table_i=ready  \rangle 
\end{align*}

%\noindent Exogenous events have preconditions. For example, it is possible to specify that when new customers arrive, they first occupy table 1 if table 1 is available, i.e. $table_1=empty$. If table 1 is occupied, then customers move to the next available table. %Similarly, customers do not place an order unless $RoboX$ is at their table and had asked them whether they would like to order, i.e. $table_i=requested$. The occurrence probabilities of the different events are obviously not easy to determine. It is however possible, given enough history data, to derive reasonably accurate values. 

%\paragraph*{Succinct Modeling}
Now, consider the following unconditional achieve requirement:
\begin{align*}
&\textbf{ReqID } req_2 \textbf{ achieve } table_1=paid 
\end{align*}

\noindent This requirement specifies that the ``payment'' state should be achieved {\it as many times as possible}. Figure~\ref{fig:scenario} shows parts of the policy computed for this domain description: it shows that $RoboX$ should move to $table_1$ and wait until customers arrive (see state $s_2$). After a customer arrives, it should ask them to order. Note that due to the chosen interleaving semantics, it could occur that the customer places an order simultaneously with the request (see the transition from $s_3$ to $s_5$). Once order is received, $RoboX$ must move to the kitchen, collect the order and then deliver the order back to the customer. %Note that Fig.~\ref{fig:scenario} does not show all the transitions for brevity. 
After the customer leaves, the strategy determines that $RoboX$ should clean the table and wait for new customers. 

This strategy arguably defines a complete behavioral model for $RoboX$. The computation of this {\it optimal} strategy only requires a description of the environment, $RoboX$'s capabilities and the definition of requirements that capture the high-level goals that should be pursued. This example thus shows that suitable modeling and choice of requirements enables {\it succinct model descriptions}, based on which complex but optimal behavioral models can be derived. This should be contrasted with an approach where behavior of the agent has to be fully specified. The former approach is obviously more powerful since it: 1) requires much less effort, 2) makes explicit the {\it rational} {\it justifying} the agent's behavior and 3) provides optimality guarantees. %The derivation of highly complex behavioral specifications from high-level succinct models is one of the most powerful features of the present approach.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{Scenario}
	\caption{Computed Strategy Example (Selected States)}
	\label{fig:scenario}
\end{figure}

\paragraph*{Requirements Prioritisation}
%\label{sec:scheduling}
%So far, only domain models with one single requirement were discussed. 
When domain models include multiple requirement, the computed strategy prioritizes or schedules them according to the total reward that their satisfaction is expected to yield. For example, we extend the domain model with:
\begin{align*}
	&\textbf{ReqID } req_3 \textbf{ achieve } table_2=paid 
\end{align*}

\noindent Now, $RoboX$ has to serve $table_1$ and $table_2$. Consequently, many situations arise where $RoboX$ has to choose whether to pursue $req_2$ or $req_3$. Figure~\ref{fig:requirementscheduling} shows one of those situations: if $RoboX$ had gotten $table_1$'s order and customers at $table_2$ have not ordered yet, should it pass the order of $table_1$ to the kitchen or wait and get $table_2$'s order first? The optimal action in this case is to move to $table_2$ to get its order first before passing the two orders to the kitchen. Notice that this is indeed the optimal course of action according to the model description which specifies that $table_2$ is very likely to place an order. 


Notice that {\it prioritisation} situations, similar to the one just discussed, do not have to be identified and resolved separately, as would be required when the behavior of the system is explicitly specified. A second benefit of our requirements-driven approach is that conflict resolution is {\it optimal} according to the domain model.


\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{requirement_scheduling}
	\caption{Requirement Prioritisation/Scheduling}
	\label{fig:requirementscheduling}
\end{figure}

\paragraph*{Requirements Tradeoffs}
\label{sec:requirements_tradeoffs}
When requirements have deadlines, i.e. must be complied with within a finite number of time units, scheduling/prioritisation may not be possible. Notice that without deadlines, some requirements could remain unsatisfied indefinitely. We currently identify those situations by inspecting the generated strategies. The automation of the detection of those cases is left for future work. %A future extension of this work is thus the identification of {\it desirable properties} of strategies, i.e., properties that {\it good} strategies should satisfy, automate checking of those properties and developing techniques that can be used to {\it fix} requirements when strategies do not meet the desired properties. When requirements have deadlines, their satisfaction may conflict. 
Now, consider the following requirements:
\begin{align*}
	&\textbf{ReqID } req_4 \textbf{ achieve } table_1=delivered  \textbf{ within } 8 \\
	&\hspace{0.5cm} \textbf{ if } order_1=ready \textbf{ reward } 1000\\		
&\textbf{ReqID } req_5 \textbf{ achieve } table_2=empty \textbf{ within } 2 \\
&\hspace{0.5cm} \textbf{ if } order_2=paid \textbf{ reward } 500
\end{align*}


\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Tradeoffs}
	\caption{Requirements Trade-offs}
	\label{fig:tradeoffs}
\end{figure}
\noindent Figure~\ref{fig:tradeoffs} shows the optimal actions for seven of the possible states. They show the following features of computed strategies:

\textit{Proactive behavior:} In $s_0$, $RoboX$ does not have requirements that are {\it active} or {\it in force}. It however anticipates the activation of $req_5$ which have to be satisfied within 2 time steps. Therefore, the optimal action is to move to $table_2$ (see the states $s_0$-$s_2$). 

\textit{Disciplined Trade-offs:} Consider the situation in state $s_6$: $RoboX$ is at $table_2$, it has to clean $table_2$ (requirement $req_5$ is active) but at the same time $table_1$'s food is ready (requirement $req_4$ is active). In this case, the optimal action is to abandon the satisfaction of $req_5$ since it conflicts with the satisfaction of $req_4$, which reward is higher. Note that the collection and delivery of food starting from $table_2$ takes 8 time units, the exact time specified in the deadline of $req_4$. Hence, $RoboX$ cannot satisfy both requirements.  


%
%
%\comments{
%\subsection{Discussion}
%\label{sec:Discussion}
%This section evaluated the use of \react through a number of use cases illustrating the different features of the language. Below is a list of key points:
%\begin{itemize}
%	\item Succinct models: one main advantage of the approach is its succinct encoding of the problem since one has to describe the available capabilities in the system, the environment and the requirements. Operationalization of requirements comes from the computation of strategies on the basis of domain models. Although it does require some experience to correctly model the domain, this has to be contrasted to the effort necessary to fully and explicitly specify the behavior of the autonomous system. Furthermore, the latter does not guarantee the optimality of the specified behavioral model. 
%	\item Setting of model parameters: in some situations, the choice of the model parameters, namely requirement rewards and probabilities, may not be obvious. There are two ways which could be used to tackle this: 1) the use of reinforcement learning to adjust and learn the model parameters at runtime, 2) rely on historical data to derive values for the model parameters. Those are areas which we extend to explore in future work.
%	\item Identification of requirements: the correct identification of requirements is obviously necessary to derive correct behavioral model. One main benefit of our approach is that it enables the use of goal modeling techniques which has been proven to be reliable over the years to identify requirements \cite{Lapouchnian2005,VanLamsweerde2009,Yu2011a}.
%\end{itemize}
%
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{MDPSolutionTime}
%	\caption{MDP Solution Time}
%	\label{fig:mdp_solution_time}
%\end{figure}
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{MDPConstructionTime}
%	\caption{MDP Construction Time}
%	\label{fig:mdp_construction_time}
%\end{figure}
%}
}
\subsection{Preliminary Experimental Evaluation}
\label{sec:preliminaryeval}
We have implemented the \react framework as a Java-based prototype which uses EMFText~\cite{Heidenreich2013}, the MDPToolBox package~\cite{MDPToolbox2017} and Graphviz~\cite{Ellson2002}.
\comments{
\begin{itemize}
	\item EMFText~\cite{Heidenreich2013} is a model-based technique for the design and implementation of domain specific languages (DSLs) based on the Eclipse Modeling Framework (EMF) and its underlying modeling language Ecore. EMFText is used to define the meta-model and textual representation ({\it concrete syntax}) of \react presented in Section~\ref{sec:model_language};
	\item MDPToolBox package~\cite{MDPToolbox2017} provides classes and functions for the resolution of discrete-time MDPs in MATLAB. %The current implementation uses the {\it mdp\_policy\_iteration} function provided by MDPToolBox to solve the (constructed) MDPs;
	\item Graphviz is used for the visualization of the constructed MDP models and their solutions, i.e., the computed strategies, enabling the manual inspection and verification of adaptation strategies. The identification of properties of sound adaptation strategies and the automation of their verification represents future work.
\end{itemize}
}
There are at least two main use cases of the framework:
%\begin{itemize}
	\paragraph*{At design-time} the textual editor generated by EMFText can be used to define \react models. The corresponding MDP models and optimal strategies can be then visualized and inspected by a system designer and/or used to synthesize optimal controllers for the target autonomous systems;
	\paragraph*{At runtime} the \react Java API can be used to create instances of the \react model and the computation of optimal strategies at runtime. At runtime, strategies should be recomputed after change in either 1) requirements or 2) domain descriptions. The former generally denotes a change in system objectives or their priorities. On the other hand, the latter is needed if new information (possibly based on interactions with the environment) shows that model parameters need to be revised. There are some limitations to this use scenario which are discussed in Section~\ref{sec:limitations}.%Issues such as how and when to update runtime models represent future work.  
%\end{itemize}

Figures~\ref{fig:mdp_construction_time} and \ref{fig:mdp_solution_time} show the MDP construction and solving time for different state space sizes, respectively. It is clear from the figures that the current implementation suffers from the state explosion problem. However, the support of thousands of states is typically sufficient for a large number of problems. Furthermore, solving an MDP is a one-time effort, i.e. once an MDP is solved (given a set of requirements), the computed strategies can be used until either requirements or the domain model change.%, like other model checking and formal verification approaches. %However, there exist implementations and optimization techniques that can improve significantly the performance and support of large state spaces (see for example PRISM~\cite{Kwiatkowska2004,Kwiatkowska2011}). %\bashar{the reader may wonder why you did not use PRISM}. Note that we did not use PRISM due to MDP limitations discussed in Section~\ref{sec:mdp_overview}
%\npaola{Check the following sentence and if it is not right delete it, but extend your original one}
The improvement of the performance of our current prototype represents future work. %as follows: 1) optimize algorithms and data structures used to construct MDPs %and generate explicit MDP representations from \react models (Section~\ref{sec:mdp_construction}), 2) compute optimal strategies using the state-of-the-art probabilistic model-checker STORM~\cite{Dehnert2017}. STORM's  performance results and their comparison with those of other probabilistic model-checkers can be found in~\cite{storm_results}. %Note that we have not used PRISM or any other optimized tools because basic MDPs have the limitations identified in Section~\ref{sec:mdp_overview}. Our proof of concept implementation has the objective of showing the applicability of the proposed approach. In the future, we plan to exploit existing tools and optimization techniques by enriching them to use the extended MDPs we have introduced.

\begin{figure}
	\centering
	\begin{minipage}{.5\linewidth}
		\centering
	\includegraphics[width=\linewidth]{MDPConstructionTime}
		\caption{MDP Construction}
		\label{fig:mdp_construction_time}
	\end{minipage}%
	\begin{minipage}{.5\linewidth}
		\centering
	\includegraphics[width=\linewidth]{MDPSolutionTime}
		\caption{MDP Solution}
	\label{fig:mdp_solution_time}
	\end{minipage}
\end{figure}


%Therefore, the focus of this section is to illustrate the various capabilities of the framework through a number of examples. In the following, for clarity, the computed strategies for the examples are not presented in full. Rather, few states are selected and their corresponding {\it optimal} actions are discussed. 





==> Submission Arxiv/Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Autonomous systems such as unmanned vehicles and robots play an increasingly relevant role in our societies. %Therefore, there is a need for methods and frameworks to simplify the design, development and maintenance of those highly complex systems~\cite{Salehie2009,Cheng2009a,Lemos2011}.
%The complexity of autonomous systems arises from many factors. 
Many factors contribute to the complexity in the design and development of those systems. First, they typically operate in dynamic and uncontrollable environments~\cite{Salehie2009,Cheng2009a,Lemos2011,Esfahani2013,Moreno2015}. Therefore, they must continuously adapt their configuration in response to changes, both in their operating environment and in themselves. Since the frequency of change cannot be controlled, decision-making must be almost instantaneous to ensure timely responses. %Moreover, adaptations should be driven by {\it optimal} with respect to goals of the system. 
From a design and management perspective, it is desirable to minimize the effort needed to design the system and to enable its runtime updating and maintenance. %It has therefore been advocated that systems should be requirements-aware~\cite{Sawyer2010}.
%Several proposals have made to deal with aforementioned challenges. 

A promising technique to address those challenges is requirements-driven adaptation that endow systems with the necessary means to {\it autonomously} operate based on their requirements. Requirements are prescriptive statements of intent to be satisfied by cooperation of the agents forming the system~\cite{Lamsweerde2009}. They say what the system will do and not how it will do it~\cite{Zave1997}. Hence, software engineers are relieved from the onerous task of prescribing explicitly how to adapt the system when changes occur. %Furthermore, this enables to benefit from techniques for requirements elicitation, refinements and analysis  developed in Requirements Engineering (RE)~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017}.
%Several proposals have made to deal with aforementioned challenges. 
Many current requirements-driven adaptation techniques~\cite{Calinescu2010,Filieri2016} %combine Quantitative Runtime Verification (QRV)~\cite{Calinescu2010,Filieri2016} with 
follow the Monitor-Analyze-Plan-Execute-Knowledge (MAPE-K) paradigm~\cite{Kephart2003}, which usually works as follows~\cite{Weyns2017}: the {\it Monitor} monitors the {\it managed system and its environment}, and updates the content of the {\it Knowledge} element accordingly; the {\it Analyse} activity %, sometimes using probabilistic model-checking, 
 uses the up-to-date knowledge to determine whether there is a need for adaptation of the managed element according to the adaptation goals that are available in the knowledge element. If adaptation is required, the {\it Plan} activity puts together a plan that consists of one or more adaptation actions. The adaptation plan is then executed by the {\it Execute} phase. 

This approach %is suitable only when the frequency of change is low and when adaptations are instantaneous, i.e., the new configuration can be immediately deployed. Otherwise, this approach 
has two main limitations in highly-dynamic operational environments. First, it tends to be myopic since the system adapts in response to changes without anticipating what the subsequent adaptation needs will be~\cite{Moreno2015} and, thus, it does not guarantee the optimality of the {\it overall behavior} of the autonomous system. This is particularly crucial for systems that have to operate continuously without interruption over long periods of time, e.g., cyber-physical systems. Second, the time to plan adaptations could make timely reaction to changes impossible, particularly in fast changing environments. Therefore, an approach that enables an almost instantaneous reactions to changes is needed. %Those limitations are further elaborated on an example in Sec.~2. 

%To compute optimal strategies or verify satisfaction of requirements, many current  frameworks and techniques propose to encode adaptation problems using general-purpose modeling languages such as those integrated in state-of-the-art probabilistic model checkers, i.e. PRISM and STORM. We argue that this approach does not allow natural and intuitive specification of many adaptation problems. In particular, the primitives of those languages, typically state variables, transition and reward functions, are far from the basic entities of autonomous systems, i.e. the system, environment, capabilities and requirements. To address this mismatch, we advocate the development of Domain-Specific Models and Languages (DSML) tailored to the characteristics and nature of adaptation problems for autonomous systems and to support all basic entities of autonomous systems as first-class entities in the DSML. 


%This is to be contrasted with current approaches where software engineers have to adapt to their problem to a general-purpose language which primitives do not match those of the problem at hand. Indeed, to encode requirements in languages that are currently supported by state-of-the-art model checkers, software engineers have to find a way to encode adaptation problems in terms of state variables, transition and reward functions, primitives that are not adequate nor advocate the succinct nor intuitive problem definition.


%combine Quantitative Runtime Verification (QRV)~\cite{Calinescu2010,Filieri2016} with the Monitor-Analyze-Plan-Execute-Knowledge (MAPE-K) paradigm. This usually works as follows~\cite{Weyns2017}: the {\it Monitor} monitors the {\it managed system and its environment}, and updates the content of the {\it Knowledge} element accordingly; the {\it Analyse} activity, sometimes using probabilistic model-checking, uses the up-to-date knowledge to determine whether there is a need for adaptation of the managed element according to the adaptation goals that are available in the knowledge element. If adaptation is required, the {\it Plan} activity puts together a plan that consists of one or more adaptation actions. The adaptation plan is then executed by the {\it Execute} phase. 

%This approach has two main limitations in highly-dynamic operational environments. First, it tends to be myopic since the system adapts in response to changes without anticipating what the subsequent adaptation needs will be~\cite{Moreno2015} and, thus, it does not guarantee the optimality of the {\it overall behavior} of the autonomous system. This is particularly crucial for systems that have to operate continuously without interruption over long periods of time. Second, the time necessary to plan adaptations could make impossible to react in a timely manner to changes, particularly in fast changing environments. Therefore, an approach that enables an almost instantaneous reaction to changes is needed. %Those limitations are further elaborated on an example in Sec.~2. 



%Several proposals have made to deal with aforementioned challenges. 
%Many current adaptation techniques combine Quantitative Runtime Verification (QRV)~\cite{Calinescu2010,Filieri2016} with the Monitor-Analyze-Plan-Execute-Knowledge (MAPE-K) paradigm. This usually works as follows~\cite{Weyns2017}: the {\it Monitor} monitors the {\it managed system and its environment}, and updates the content of the {\it Knowledge} element accordingly; the {\it Analyse} activity, sometimes using probabilistic model-checking, uses the up-to-date knowledge to determine whether there is a need for adaptation of the managed element according to the adaptation goals that are available in the knowledge element. If adaptation is required, the {\it Plan} activity puts together a plan that consists of one or more adaptation actions. The adaptation plan is then executed by the {\it Execute} phase. 

%This approach has two main limitations in highly-dynamic operational environments. First, it tends to be myopic since the system adapts in response to changes without anticipating what the subsequent adaptation needs will be~\cite{Moreno2015} and, thus, it does not guarantee the optimality of the {\it overall behavior} of the autonomous system. This is particularly crucial for systems that have to operate continuously without interruption over long periods of time. Second, the time necessary to plan adaptations could make impossible to react in a timely manner to changes, particularly in fast changing environments. Therefore, an approach that enables an almost instantaneous reaction to changes is needed.

%From a system design and maintenance perspective, many adaptation frameworks do not separate between computational and system design models. We argue that this makes it harder to properly design the system. 

%In contrast, approaches that aim at optimizing the system behavior are {\it proactive} in the sense that they take into account not only the current conditions, but how they are estimated to evolve, improving the outcome of adaptation~\cite{Camara2014a}.

%The reference architecture for realising the functions of self-adaptive systems is the Monitor-Analyze-Plan-Execute-Knowledge (MAPE-K) paradigm~\cite{Weyns2017}. MAPE-K is a continuous process where the {\it Monitor} element acquires data from the managed element and its environment, and processes this data to update the content of the {\it Knowledge} element accordingly. The {\it Analyse} element uses the up-to-date knowledge to determine whether there is a need for adaptation of the managed element according to the adaptation goals that are available in the knowledge element. If adaptation is required, the {\it Plan} element puts together a plan that consists of one or more adaptation actions. The adaptation plan is then executed by the {\it Execute} element that adapts the managed element as needed. 

%use the Monitor Analyze Planning Execute (MAPE):  paradigm where classical planning (see for example STRIPS~\cite{Fikes1971} PDDL~\cite{mcdermott98pddl}) is used to determine the best course of action when a change is detected. This reactive paradigm is inadequate, unless the computation of plans is instantaneous. For example, imagine if while $RoboX$ is moving to serve a customer in the dining room, a weak battery signal is detected. In this case, it is possible to halt the execution of the plan until a new plan is computed or resume the execution of the current plan with no guarantees of its optimality. If the frequency of changes detected in the environment is high, then this situation is worsened as the autonomous system would be permanently stuck in a state where it is computing plans without acting, or it would be indefinitely pursuing plans with no guarantees of their optimality. The computation of an {\it optimal strategy} provides a solution to this problem. An optimal strategy identifies the best adaptation action that should be taken in every possible evolution of the system. Thus, it enables an almost instantaneous response to every possible change since optimal responses are precomputed, eliminating the need to re-plan after every change\paola{I don’t think it is clear how this guarantee instantaneous respone }. In other words, the computation of a strategy defines a {\it reflex controller} for the autonomous system that enables it to optimally and instantaneously react to every possible future change.
In this paper, we propose the Optimal by Design (\react) framework as a first step towards dealing with the aforementioned challenges. 
\react supports a model-based approach to simplify the high-level design and description of autonomous systems, their capabilities, requirements and environment. Based on these high-level models, \react constructs a Markov Decision Process (MDP) that can then be solved (possibly using state-of-the-art probabilistic model checkers) to produce optimal {\it strategies} for the autonomous system. These strategies define {\it optimal reflex} controllers that ensure the ability of autonomous systems to behave optimally and almost instantaneously to changes in itself or its environment. 

Several previous works~\cite{Camara2014a,Camara2015,Moreno2015,Camara2016} encode adaptation problems using general-purpose languages such as those proposed by probabilistic model checkers, e.g., PRISM~\cite{Kwiatkowska2011}. Unfortunately, these languages do not offer primitives tailored to the design and analysis of autonomous systems. This makes them unsuitable to adequately describe the software requirements~\cite{Lamsweerde2009} of the autonomous system and the environment in which it operates. Examples of limitations of these languages resolved in this paper through \react are the Markovian assumption~\cite{Bacchus96} and the implicit-event model~\cite{boutilier99}. 

 %\react clearly separate between the autonomous system model and the underlying computational paradigm, namely MDP. More precisely, 
In a nutshell, \react introduces a novel Domain Specific Modeling Language (DSL) for the description of autonomous systems, its environment and requirements. The semantics of the DSL is then defined in terms of a translation into a Markov Decision Process (MDP) model to enable the synthesis of optimal controllers for the autonomous system. This separation between the model (i.e. the DSL) and its underlying computational paradigm (i.e. MDP), brings several important advantages. First, the level of abstraction at which systems have to be designed is raised, simplifying their modeling by software engineers. Second, requirements become first-class entities, making it possible to elicit them using traditional requirements engineering techniques~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017} and to benefit from goal refinement, analysis and verification techniques developed for goal modeling languages. Moreover, this approach clarifies the limitations of the underlying computational model, namely the aforementioned Markovian assumption and the implicit-event model, and permits the identification and implementation of extensions necessary to overcome those limitations and support the required analysis, verification and reasoning tasks. 

%We argue that this approach does not allow natural and intuitive specification of many adaptation problems. In particular, the primitives of those languages, typically state variables, transition and reward functions, are far from the basic entities of autonomous systems, i.e. the system, environment, capabilities and requirements. To address this mismatch, we advocate the development of Domain-Specific Models and Languages (DSML) tailored to the characteristics and nature of adaptation problems for autonomous systems and to support all basic entities of autonomous systems as first-class entities in the DSML. \react clearly separate between the autonomous system model and the underlying computational paradigm, namely MDP. This has several important advantages. First, the level of abstraction at which systems have to be designed is raised, simplifying their modeling by software engineers. Second, requirements become first-class entities, making possible to elicit them using traditional requirements engineering techniques~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017} and to benefit from goal refinement, analysis and verification techniques developed for goal modeling languages. Moreover, this approach clarifies the limitations of the underlying computational model and simplifies the identification of extensions needed to support required analysis, verification and reasoning tasks. For example, this paper identifies and resolves two MDP limitations, namely the Markovian assumption~\cite{Bacchus96} and the implicit-event model~\cite{boutilier99}, to enable the computation of optimal strategies based on autonomous systems requirements. 

 

%One salient feature of \react is that it allows to combine the benefits of both techniques developed for the elicitation, refinement and analysis of requirements developed around goal modeling frameworks~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017}, and from the vast amount of research around Markov Decision Process and its various extensions and tools. 


The remainder of this paper is structured as follows. Section~\ref{sec:running_example} presents a motivating example, which will be used as a running example throughout the paper. Section~\ref{sec:framework_overview} presents an overview of the \react framework. Section~\ref{sec:model_language} introduces the framework's model and language. Section~\ref{sec:controller_synthesis} provides the semantics of \react models by presenting their translation into MDPs. Section~\ref{sec:evaluation}presents an evaluation of the framework. Section~\ref{sec:limitations} discusses limitations and threats to validity. Finally, Section~\ref{sec:related_work} discusses related work and Section~\ref{sec:conclusion} concludes the paper and presents future work.

==> Submission Arxiv/Limitations.tex <==
\section{Limitations \& Issues}
\label{sec:limitations}
This section discusses the current limitations and issues related to using \react and means to address them.
\paragraph*{Setting of Model parameters} determining probabilities of actions and events can be challenging. We envisage that they shall be computed by adapting existing techniques that enable computation and learning of model parameters at runtime. For example, we could use~\cite{Epifani2009} where Bayesian techniques are used to re-estimate probabilities in formal models such as Markov chains based on real data observed at runtime; or~\cite{Calinescu2014} which proposes an on-line learning method that infers and dynamically adjusts probabilities of Markov models from observations of system behaviour. Alternatively, reinforcement learning techniques~\cite{Tesauro2007} could be used. %Alternatively, we can rely on reinforcement learning, e.g., to learn the values of model parameters during operation. %Those areas represent future work.
	
\paragraph*{Identification of requirements} strategies are computed according to requirements. It is thus crucial that they be correctly identified. \react supports traditional goal modeling techniques~\cite{Lapouchnian2005,VanLamsweerde2009,Yu2011a}. Those techniques have been proven reliable over the years in ensuring correct elicitation, refinement, analysis and verification of requirements~\cite{Lapouchnian2005,VanLamsweerde2009,Yu2011a}. 
	
	\paragraph*{Suitability of the Application Domain} it is necessary to identify system conditions under which the framework may be used. Towards answering this question, we first define a predictable (unpredictable) system as one where probabilities of occurrence and effects of events/actions do not (do) change with time. Similarly, we define a dynamic (erratic) system as one where the rate of {\it relevant}\footnote{A change is relevant if it renders computed strategies obsolete.} change in those probabilities is within the order of hours or days (minutes or seconds). Our current prototype implementation computes strategies within minutes. Consequently, we conjecture that it supports the runtime synthesis of controllers in predicable and unpredictable dynamic systems. Erratic systems are not supported. A more precise definition of those limitations represents future work.  



%When used at runtime, the re-computation of new controllers is triggered by change in either 1) requirements or 2) domain descriptions. Change in requirements is generally triggered by a change in system objectives or their priorities. On the other hand, change in other entities of the domain descriptions is needed if information (possibly based on interactions with the environment) shows that action and event descriptions need to be revised. 

%We will distinguish between predictable/unpredictable and dynamic/erratic systems as follows: system predictability (unpredictability) means that probabilities of occurrence and effects of events/actions could be unknown but do not (do) vary with time. We define a dynamic (erratic) system as one where the rate of relevant change in these probabilities is within the order of hours or days (minutes or seconds). Since our current prototype computes strategies within minutes, it is perfectly capable of supporting predicable and unpredictable dynamic systems. It does not support however control of erratic systems. We plan to investigate further runtime issues such as when it is {\it necessary} to compute new controllers and to identify more precisely the limitations of the framework with respect to the frequency and rate of change.




==> Submission Arxiv/Overview.tex <==
\section{\react Modeling Language}
\label{sec:model_language}
%The computation of {\it optimal strategies} is based on a {\it domain model}. A domain model specifies the environment, the capabilities of the autonomous system (or agent) and its requirements. %A strategy, as opposed to a plan which produces a finite course of actions, defines an optimal behavior. Effectively, the computation of a strategy specifies a {\it reflex} controller for the autonomous system that is able to decide optimally and instantly which action to execute in every possible foreseeable situation.

%For the definition of requirements, \react provides a set of templates. Those templates correspond to different typical requirement types. This approach provides several advantages: (1) it simplifies the expression and interpretation of requirements\footnote{This should be contrasted with an approach where requirements have to be specified using temporal logic formulae.}, (2) supports their maintainability and modification, and (3) simplifies their analysis and verification. Furthermore, this approach makes it possible to integrate REact with goal modeling frameworks such as KAOS~\cite{VanLamsweerde2009} and i*~\cite{Yu2011a}. This makes it possible to benefit from the refinement, analysis and elicitation techniques developed for these frameworks.




%An {\it action} is a particular type of event instigated by an agent (e.g., $RoboX$) in order to change the system's state. The agent has control over what actions are taken and when, though the effects of taking an action might not perfectly predictable. In contrast, {\it exogenous events} are not under the agent's control, and their concurrency may be only partially predictable. 



==> Submission Arxiv/ReactOverview.tex <==
\section{Framework Overview}
\label{sec:framework_overview}
\react is a framework for the model-based requirements-driven synthesis of optimal adaptation strategies for autonomous systems. The model-based approach raises the level of abstraction at which systems need to be described and simplifies model maintenance and update. Adaptation in \react is {\it requirements-driven}, enabling systems to autonomously determine the best way to pursue their objectives. %, as opposed to following hard-coded predefined rigid adaptation plans. %Requirements are prescriptive statements of intent to be satisfied by cooperation of the agents forming the system~\cite{Lamsweerde2009}. They say what the system will do and not how it will do it~\cite{Zave1997}. 
%Hence, software engineers are relieved from the onerous task of prescribing explicitly the strategies that are needed to adapt the system when changes occur. This also enables \react to benefit from techniques for the elicitation, refinements and analysis of requirements developed in Requirements Engineering (RE)~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017}\paola{why?}. 
Based on \react models, Markov Decision Processes (MDPs) are constructed. Solving those MDPs determines the system's optimal strategy, i.e., the  behavior that maximizes the satisfaction of requirements. In a strategy, the best adaptation action that should be taken in every possible (anticipated) future evolution of the system is identified, eliminating the need to re-analyze and re-plan after every change and enabling almost instantaneous reactions. Indeed, an optimal strategy defines a {\it reflex controller} that can react optimally and in a timely way.

Figure~\ref{fig:react_overview} depicts an overview of the framework, which includes a model (and a language) to describe the basic elements of self-adaptive systems~\cite{Weyns2017}: the {\it environment} refers to the part of the external world with which the system interacts and in which the effects of the system will be observed and evaluated; the {\it requirements} or adaptation goals are the concerns that need to be satisfied; the {\it managed system} represents the application code or capabilities/actuators that can be leveraged to satisfy the requirements. Based on these elements, the {\it controller} or the managing system ensures that the adaptation goals are satisfied in the managed system, is synthesized.


\begin{figure}
	\centering
	\includegraphics[width=0.92\linewidth]{REact_Overview}
	\caption[Restaurant Layout]{Framework Overview}
	\label{fig:react_overview}
\end{figure}

\comments{
From an engineering perspective, \react can be integrated into the architecture proposed by Kramer and Magee's for the engineering of self-adaptive software systems [31]. Their architecture comprises of three layers~\cite{Weyns2017}: (1) the bottom layer (the component layer) consists of the interconnected components that provide the functionalities of the system, (2) a middle {\it change management} layer which consists of a set of pre-specified plans. The middle layer reacts to status changes of bottom layer by executing plans with change actions that adapt the component configuration of the bottom layer. The middle layer is also responsible for effecting changes to the underlying managed system in response to new objectives introduced from the layer above. (3) The top layer, {\it Goal Management}, comprises a specification of high-level goals. This layer produces change management plans in response to requests for plans from the layer beneath or after new goals are introduced by stakeholders. REact can be integrated in this architecture as follows: the {\it goal management} layer would comprise REact domain models which would be translated into MDPs. Solving those MDPs would generate the {\it change management} layer or the plans for reacting to changes at the bottom layer. A request for a new set of plans, or in other words the computation a new strategy, would be produced by the change management layer whenever there is a need to update the models of the component layer or of the environment, or after the introduction of new system goals or requirements by stakeholders.

One important benefit of this approach is that relying on requirements for the generation of strategies makes possible to benefit from works on requirements elicitation, refinements and analysis produced over the years in Requirements Engineering (RE)~\cite{Lamsweerde2009,Sawyer2010,Whittle2010,Morandini2017}. It also enables to benefit from the powerful computational machinery that comes with Markov Decision Models and its extensions and tools.


The software of an autonomous robot such as $RoboX$ must satisfy various requirements. First, it must 

enable it to satisfy its various goals and requirements. For example, after getting an order, $RoboX$ must also ensure that the order is given to the kitchen and that subsequently food is delivered to the table. It may also need to charge its batteries after a low battery signal is detected. Obviously, these requirements may conflict. Therefore, $RoboX$ must be endowed with the intelligence necessary to optimize the satisfaction of its various (possibly conflicting) requirements according to the present situation.

There are several ways to define a controller for $RoboX$. One possibility is to predefine all possible situations and specify how the robot should behave in each. This solution is impractical as there are potentially millions of situations which would need to be covered. To rely on the Monitor Analyze Planning Execute (MAPE-K) paradigm could be a better alternative: the robot monitors the environment, plans its best course of action accordingly and then executes the plan. However, the use of planning has some shortcomings. For example, it is not suitable for handling of uncertainty during plan execution. For example, if while the robot is executing some plan, a customer places an order, should the current plan be abandoned or resumed? If the robot decides to resume the plan, then it might be pursuing a sub-ideal plan. On the other hand, if it decides to recompute its plan, then frequent occurrences of events in its environment may prevent it from executing any plan altogether. Furthermore, actuators of $RoboX$ may not be perfect and may not necessary always produce their desired effects. For example, it could be the case that moving to the kitchen from the dining room may sometimes fail, due to the movement of customers in the restaurant. 

Besides dealing with uncertainty, there is the need to deal with multiple (possibly conflicting) requirements. For example, this may happen if $RoboX$ should charge its batteries and bring food to a customer's table while it is still hot. There is therefore a need to support disciplined trade-off of requirements that is based on reasoning about the importance of requirement satisfaction. In order to do so, there should be a reward or utility function which specifies the expected return or payoff for requirements satisfaction and $RoboX$ should choose its actions such that they maximize  this reward or utility function. 

Thus, to deal with the aforementioned challenges, the software of $RoboX$ should aim at the {\it optimal} satisfaction of its {\it requirements}~\cite{Zave1997,Lamsweerde2009} given a description consisting of the system and its environment. Notice that requirements say what the system will do and not how it will do it~\cite{Zave1997}. Thus, they enable to raise the level of abstraction of system specifications and reduce considerably the size of system specifications that have to be provided. 

To identify the optimal behavior of the system based on a high-level description of the system, its environment and its requirements, we construct a Markov Decision Process (MDP). By solving this MDP, we can compute an {\it optimal} strategy that identifies the action that should be taken in every possible situation in order to best satisfy the requirements of $ROboX$. 


}


==> Submission Arxiv/RelatedWork.tex <==
\section{Related Work}
\label{sec:related_work}

\begin{table}[t]
	\caption{Comparison of \react with Related Frameworks}
	\label{tab:comparison_table}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline 
		{\bf Comp.}    		 & Sub-criteria	&$F_1$&$Q_1$&$K_1$&$R_1$&$K_2$&$A_1$&$R$\\
		\hline	 
		\multirow{3}{*}{Model}       & Requirements &\yes &\yes &\yes &\yes &\yes &\yes  &\yes  \\
									 & Capabilities &\yes &\ps  &\yes &\ps  &\ps  &\ps  &\yes \\
								 	 & Events       &\no  &\ps  &\no  &\no  &\ps  &\no  &\yes \\
		
		\hline 	 
		\multirow{2}{*}{Uncert.}     & Occurrence   &\no  &\ps  &\no  &\no  &\ps  &\no  &\yes \\
								     & Effects      &\no  &\ps  &\no  &\yes &\ps  &\no  &\yes \\
		\hline 
		\multirow{3}{*}{Adapt  }     & Explicit     &\yes &\na  &\yes &\yes &\na  &\yes  &\na  \\
									 & Configuration&\na  &\yes &\na  &\na  &\yes &\na &\na  \\									
									 & Behavior     &\na  &\na  &\na  &\na  &\na  &\na  &\yes \\
		
		\hline 
		\multicolumn{9}{|l|}{\yes: supported \hspace{3.3cm} \no: not supported \hspace{1cm}}\\
		\multicolumn{9}{|l|}{\ps: partially supported (implicit) \hspace{1cm} \na: not applicable}\\
		\hline
		%\multicolumn{5}{|l|}{$R_1$: RELAX~\cite{Whittle2010}}\\
		%\multicolumn{5}{|l|}{$T_1$: Tropos4AS~\cite{Morandini2017}}\\
		\multicolumn{9}{|l|}{$F_1$: FLAGS~\cite{Baresi2010}\hspace{0.5 cm}$Q_1$: QoSMOS~\cite{Calinescu2010}\hspace{0.5 cm}$K_1$: KAOS~\cite{VanLamsweerde2009,Letier2002,Cailliau2017}}\\
		%\multicolumn{7}{|l|}{$G_1$: GODA~\cite{VanLamsweerde2009,Letier2002,Cailliau2017}}\\
		%\multicolumn{5}{|l|}{$A_1$: ADAM~\cite{Ghezzi2013}}\\
		%\multicolumn{9}{|l|}{$F_1$: FLAGS~\cite{Baresi2010}}\\
		%\multicolumn{5}{|l|}{$P_1$: POISED~\cite{Esfahani2011}}\\
		%\multicolumn{5}{|l|}{$F_2$: FUSION~\cite{Elkhodary2010}}\\
		%\multicolumn{9}{|l|}{$Q_1$: QoSMOS~\cite{Calinescu2010}}\\
		\multicolumn{9}{|l|}{$R_1$: Rainbow~\cite{Garlan2004,Cheng2012}\hspace{2.3cm}$K_2$: KAMI~\cite{Filieri2012m}}\\
		%\multicolumn{5}{|l|}{$C_1$: Camara~\cite{Camara2015}\\
		%\multicolumn{9}{|l|}{$K_1$: KAMI~\cite{Filieri2012m}}\\
		\multicolumn{9}{|l|}{$A_1$: ActivFORMS~\cite{Iftikhar2014}\hspace{2.35cm}$R$: \react}\\
		%\multicolumn{9}{|l|}{$M_1$: GM\_al~\cite{Moreno2015,Camara2016}}\\
		
		%\multicolumn{5}{|l|}{$R_2$: Calinescu and Kwiatkowska 09~\cite{}}\\
		%\multicolumn{5}{|l|}{$R_2$: Li et al 14 controller synthesis~\cite{}}\\
		%\multicolumn{5}{|l|}{$A_1$: ActiFORMS 09~\cite{}}\\
		%				\multicolumn{5}{|l|}{$R_2$: Emami-Taba et al 15 controller synthesis~\cite{}}\\
		\hline
	\end{tabular}
\end{table}

%Research on autonomous and self-adaptive systems covers a wide range of topics, which include models and languages for the expression and specification of requirements~\cite{Cheng2009,Whittle2010,Cheng2012}, analysis and verification techniques~\cite{Mendonca2016}, adaptation architectures~\cite{Kephart2003,Garlan2004,Braberman2015}, etc. This paper introduces a model-based approach for the requirements-driven synthesis of optimal adaptation strategies for autonomous systems. The focus of this section will therefore be on self-adaptation frameworks and techniques. 
Table~\ref{tab:comparison_table} compares the features of \react with some notable requirements-driven adaptation frameworks according to the criteria in Sec.~\ref{sec:running_example}, divided along the following dimensions.%\bashar{The table does not suffice you need at the very least summarize the table in text and help the reader interpret it. }

\textit{Modeling} compares the frameworks with respect to their support of the explicit modeling and representation of requirements, capabilities and events. Those feature are desirable as they simplify system design, its maintenance and modularity. %For example, consider implicit-event models where the system designer has to determine the probabilities of transitions resulting from the simultaneous occurrence of adaptation actions and exogenous events. %This feature corresponds to the need to support of a model-based-requirements-driven adaptation as discussed in Sec.~\ref{sec:running_example}. 

\textit{Uncertainty} compares the support of uncertainty in exogenous event occurrences and effects. %Those features are motivated and discussed in Sec.~\ref{sec:running_example}.
%\npaola{I am noticing that you are not dealing with probabilistic vs fuzzy approaches even though FLAGS is fuzzy based}

\textit{Adaptation} compares the type of adaptation strategies, which can be explicitly defined, configuration selection or behavior optimization. Configuration selection is a reactive approach where, after requirements are violated, the alternative system configurations are compared and the best one is selected. %means that Two types of automated adaptation are distinguished: selection of the optimal system's parameters/configuration in light of the current conditions. %Typically, parameters/configuration optimization is performed by monitoring the system requirements and, upon the detection of a violation of system requirements, the possible alternative configurations are compared and the one which maximizes the satisfaction of requirements is selected. %This reactive approach is only suitable when adaptations are instantaneous, otherwise it tends to be myopic since the system adapts in response to changes without anticipating what the subsequent adaptation needs will be~\cite{Moreno2015}. 
%Typically, this is a reactive approach where adaptation is triggered after violation of requirements. 
Behavior optimization is a proactive approach which takes into account not only the current conditions, but how they are estimated to evolve~\cite{Camara2014a}. %More precisely, 
Only behavior-based optimization supports the two requirements of (1) proactive and long-term behavior optimization, and (2) fast and optimal response to change. Note that adaptation based on explicitly defined strategies is fast but provides no optimality guarantees.

Table~\ref{tab:comparison_table} shows that adaptations in many current frameworks are either explicitly defined~\cite{Letier2002,Garlan2004,Lamsweerde2009,Baresi2010,Cheng2012,Iftikhar2014,Cailliau2017} or determined based on a comparison of possible system configurations~\cite{Calinescu2010,Filieri2012m}, without taking into account future evolutions of the system. It also shows that explicit-event and action models are rarely considered. For example, QosMOS and KAMI consider Markov chains. This is why these frameworks have an {\it implicit} models of actions and events in Table~\ref{tab:comparison_table}. %Notice that this paper considers MDPs, which are an extension of Markov chains that incorporate non-deterministic actions: if only one action exists, a MDP reduces to a Markov chain. 
Similarly, ActivForms rely on Timed Automata and the {\it Execute} activity is explicitly defined. Therefore, ActiveForms has explicit adaptation strategies and uncertainty is not handled. 
%\paragraph{Markov Models \& Stochastic Multi-player Games} 
%The  works~\cite{Camara2014a,Camara2015,Moreno2015,Camara2016} are the closest to ours. 
In \cite{Moreno2015}, MDP is used to identify optimal adaptations at runtime, taking into account the delay or latency required to bring about the effects of adaptation tactics . In~\cite{Camara2014a,Camara2016}, latency-aware adaptation is studied using stochastic multi-player games (SMGs). %latency-aware adaptation and
In \cite{Camara2015}, SMGs are used to generate optimal adaptation plans for architecture-based self-adaptation. These works exploit PRISM and PRISM-games to solve adaptation problems. So, they have the limitations discussed in Section~\ref{sec:comparison_probabilistic_model_checkers}.


%Both MDP and SMGs support explicit modeling of uncertainty in the outcome of adaptation actions. SMGs further support the explicit modeling of the environment and events. With respect to our work, reward structures in both MDP and SMG are limited by the Markovian assumption (see Section~\ref{sec:mdp_overview}). Consequently, they do not support specification of requirements shown in Section~4.2. Moreover, in (turn-based) SMG, e.g. in~\cite{Camara2015}, nondeterministic choice at each state is resolved by the player who controls the state, i.e. at each turn, one action is chosen either by the system or the environment. In contrast, in the model of the environment considered here, {\it multiple} exogenous events can occur {\it concurrently} with every action. %Finally, we seperate 

%In contrast, we study the synthesis of optimal controllers for autonomous systems, i.e. optimization of behavior over an {\it infinite-horizon} based on explicit models of the system, its environment, capabilities and requirements. From a design perspective, we separate the design models (\react models) from the underlying computational Markov model. %the level of abstraction at which systems have to be represented and to support the construction of MDPs with non-Markovian rewards.   

Several other works~\cite{Esfahani2011,Elkhodary2010,Bencomo2013} studied the optimization of system configurations. In contrast, this paper focuses on behavior optimization. Several recent proposals explored the application of concepts from control theory~\cite{Filieri2014,Filieri2015,Shevtsov2016,Filieri2017} to perform system adaptation. One main difference with respect to these works is that their focus is on the optimization of quantifiable and measurable non-functional goals, such as response time, as opposed to behavior optimization based on functional requirements, the primary focus here.
%\paragraph{Other works} %Other adaptation frameworks were not included in Table~\ref{tab:comparison_table}. 
%Esfahani et al.~\cite{Esfahani2011} introduced $POISED$ to tackle the problem of decision making under {\it internal uncertainty}, that is the difficulty of determining the impact of adaptation on the system's quality objectives. Alkhodary et al.~\cite{Elkhodary2010} proposed the FeatUre-oriented Self-adaptatION ($FUSION$) framework to learn the impact of enabling/disabling of features on system metrics at runtime and support the runtime adaptation of the system to optimal feature configurations. Bencomo and Belaggoin~\cite{Bencomo2013} study the use of Dynamic Decision Networks for reasoning about goal models and satisfaction of softgoals. %Adaptation is initiated when a goal is violated, e.g., when the value of a metric is unacceptable. $FUSION$ then plans the adaptation by identifying the features which affects the violated goal. An {\it effect} activity then moves the system to the optimal feature configuration determined during planning. 
%The focus of these works is optimization of system configuration whereas this paper focuses on behavior optimization. 
%Several recent proposals explored the application of concepts from control theory~\cite{Filieri2017} to adapt software systems. Push-Bottom Methodology ($PBM$)~\cite{Filieri2014} constructs a linear model of the software %by testing a set of sample values of the control variables and measuring their effects on specified non-functional requirements. The synthesized model is then used 
%and uses this synthesized model to adapt the software automatically at runtime to maximize the satisfaction of a single goal. More recent frameworks such as $AMOCS$~\cite{Filieri2015} and $SimCA$~\cite{Shevtsov2016} add support of multiple goals. One main difference with respect to these works is that their focus is on the optimization of quantifiable and measurable non-functional goals, such as response time, as opposed to behavior optimization based on functional requirements, the primary focus here.


%The work on autonomous and self-adaptive systems covers a wide range of topics. Those topics include models and languages for the expression and specification of requirements~\cite{Cheng2009,Whittle2010,Dalpiaz2013}, analysis and verification techniques~\cite{Mendonca2016}, adaptation architectures~\cite{Kephart2003,Garlan2004,Braberman2015}, literature reviews~\cite{Yang2014,Shevtsov2017}, requirements monitoring~\cite{Dalpiaz2013}, research agendas and vision papers~\cite{Cheng2009a,Sawyer2010,Lemos2017,Weyns2017}, requirements operationalization and decision making under uncertainty~\cite{Esfahani2011}. Our contributions are mostly related to the modeling of autonomous systems and their requirements as well as to the synthesis of controllers for those systems. 

%It is important to notice the difference between approaches which aim at system's parameters/configuration optimization and those seeking behavior optimization. Typically, parameters/configuration optimization is performed by monitoring the system requirements and, upon the detection of a violation of system requirements, the possible alternative configurations are compared and the one which maximizes the satisfaction of requirements is selected. This reactive approach is only suitable when adaptations are instantaneous, otherwise it tends to be myopic since the system adapts in response to changes without anticipating what the subsequent adaptation needs will be~\cite{Moreno2015}. In contrast, approaches that aim at optimizing the system behavior are {\it proactive} in the sense that they take into account not only the current conditions, but how they are estimated to evolve, improving the outcome of adaptation~\cite{Camara2014a}. 

%Cheng et al.~\cite{Whittle2010} introduced RELAX, a new requirements language for self-adaptive systems. It introduces three types of operators ordinal, temporal or modal deviations to handle uncertainty, or deviations form ideal behavior at runtime. This work is extended in~\cite{Cheng2009} to support the specification of uncertainty in the objectives (the system goals).


%Dalpiaz et al.~\cite{Dalpiaz2013} introduce Runtime Goal Models (RGM) that extend Design Goal Models (DGM) to enable the monitoring and diagnosis of Runtime Goal Instances (RGI). 

%GODA (Goal-Oriented Dependability Analysis)~\cite{Mendonca2016} is a framework for reasoning about the dependability requirements of systems that operate in dynamic environments. Their approach consists of transforming a Contextual and Runtime Goal Model (CRGM), that is a design-time goal model that included goals and tasks extended with additional contextual and runtime information in a way that is consistent with the approach in~\cite{Dalpiaz2013}, into a Discrete-Time Markov Chain (DTMC). They then use PRISM to compute the probability that system goals are fulfilled. 

%Weyns and Iftikhar~\cite{Weyns2016} propose a modular approach for decision making in self-adaptive systems. They use stochastic timed automata (STA) as modeling language to represent the managed system, its environment and quality models. Simulation queries are used to determine an estimate for the value of a quality property for every possible configuration. Configurations are ranked according to the adaptation goals and the then the planner creates a plan for the highest ranked option. This plan is carried out by the Executor component. Adaptation goals are represented as a set of rules over the quality properties that are subject of adaptation. The current adaptation options list the possible configurations of the managed system. The current plan comprises the set of actions that are required to adapt the current configuration to the selected adaptation option. 

%Baresi et al~\cite{Baresi2010} proposes FLAGS, a framework that extends KAOS to allow the specification of fuzzy goals and to specify countermeasures that should be enforced when goals are violated. In comparison with REact, countermeasures can be modeled as the available actions

%Garlan et al.~\cite{Garlan2004} proposes the Rainbow framework, a reusable infrastructure that supports self-adaptation of software systems. In Rainbow, an architectural is represented as a graph where each node represents a different component. Invariants are used to specify certain properties whereas strategies define actions that should be taken when invariants are violated.   

%Esfahani et al.~\cite{Esfahani2011} introduce POISED to tackle the problem of decision making under {\it internal uncertainty}, that is the difficulty of determining the impact of adaptation on the system's quality objectives. They formulate the problem of selecting the optimal system configuration in the form of an optimization problem comprising configuration constraints, quality attributes, resources and user preferences.

%Alkhodary et al.~\cite{Elkhodary2010} introduce the FeatUre-oriented Self-adaptatION (FUSION) framework to learn the impact of enabling/disabling of features on the system metrics at runtime. Adaptation is initiated when a goal is violated, e.g., when the value of a metric is unacceptable. FUSION then plans the adaptation by identifying the features which affects the violated goal and generates an optimization problem. An effect activity then moves the system to the optimal feature configuration determined during planning.

%~\cite{B2016} The paper introduces Iterative Decision-Making Scheme (IDMS) to tackle the problem of strategy selection for an MDP with empirically determined transition probabilities and a given subset of schedulers. The authors show how IDMS can be embedded in Rainbow to extend the adaptation function of the framework, which employs a standard, point-valued MDP as its decision model. In comparison, REact computes the optimal strategy given a model of the system, the environment and requirements, as opposed to selecting a strategy from a set of already provided strategies. This work is thus complementary to ours. 

%QoSMOS~\cite{Calinescu2010} is a framework for the Management and Optimisation of the QoS of Service-Based Systems (SBS)s. It relies on and integrates into a single architecture several techniques and tools\cite{Kwiatkowska2004,Grunske2008m,Calinescu2009a,Filieri2012m}: the target system is modeled using the PRISM~\cite{Kwiatkowska2004,Kwiatkowska2007} language, the ProProST~\cite{Grunske2008m} system is used for defining the target system's QoS requirements and KAMI~\cite{Filieri2012m} is used to produce new estimates of model parameters at runtime using Bayesian estimators. Based on the system model and the state estimated by KAMI, the PRISM model checker is used to run experiments to evaluate every possible configuration of the system. The utility of those different configurations is compared and the best is selected. 

%The paper~\cite{Bencomo2013} proposes a systematic procedure to map goal models into Dynamic Decision Networks (DDN)s to support the selection of  configurations that optimizes satisficing system goals.

==> Submission Arxiv/SemanticsInprogress.tex <==
\section{Controller Synthesis}
\label{sec:controller_synthesis}
Markov Decision Processes (MDPs) are mathematical frameworks for modeling and controlling {\it stochastic dynamical systems}~\cite{boutilier99}. Informally, MDPs may be viewed as Labeled Transition Systems (LTSs) where transitions are probabilistic and can be associated to rewards. Intuitively, solving an MDP means finding an optimal {\it strategy}, i.e., determining the actions to execute in every state in order to maximize the total expected rewards. %A strategy thus effectively defines a reflex controller that can react optimally and instantly to changes in the environment of the autonomous system. 
In the following, we first introduce MDPs (Section~\ref{sec:mdp_overview}), then we discuss the main steps needed to construct an MDP starting from an \react domain model (Section~\ref{sec:mdp_construction}).



%which are defined in~\cite{boutilier99} as follows: a system that at any point in time can be in one of a number of distinct {\it states}, and in which the system's state changes over time in response to {\it events}. 

\subsection{Introduction to MDPs with Rewards}
\label{sec:mdp_overview}
A reward $MDP$ %\footnote{More precisely, a {\it stationary finite discrete-time fully-observable} MDP~\cite{Mausam2012}.}  
is a tuple $\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma \rangle$, where:
\begin{itemize}
	\item $\mathcal{S}$ is the finite set of all possible states of the system, also called the {\it state space}; %In the context of this work, a state represents a specific configuration of the autonomous system and the environment.
	\item $\mathcal{A}$ is a finite set of actions;%Actions are events that can be instigated by the agent to change the system's state.
	%\item $\mathcal{T}: \mathcal{S}\times \mathcal{A} \times \mathcal{S} \rightarrow [0, 1]$ is a transition function specifying the probability $\mathcal{T}(s_i,a,s_j)$ of going to state $s_j$ if action $a$ is executed in $s_i$. In the following, we will use the (matrix) notation $Pr_a(s_i,s_j)$ to represent $\mathcal{T}(s_i,a,s_j)$;
	
	\item $\mathcal{T}: \mathcal{S}\times \mathcal{A} \times D(\mathcal{S})$ where $D(\mathcal{S})$ is the set of probability distributions over states $S$. A distribution $d(S)\in D(S): S\rightarrow [0,1]$ is a function such that $\Sigma_{s \in S}d(s) = 1$. The transition relation $\mathcal{T}(s_i,a,d)$ specifies the probabilities $d(s_j)$ of going from state $s_i$ after execution of action $a$ to states $s_j$. In the following, we will use the (matrix) notation $Pr_a(s_i,s_j)$ to represent the probability $d(s_j)$ of going to $s_j$ after execution of $a$ in $s_i$;
	
	
	\item $\mathcal{R}: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathds{R}$ is a reward function specifying a finite numeric reward value $\mathcal{R}(s_i,a,s_j)$ when the system goes from state $s_i$ to state $s_j$ as a result of executing action $a$. Thus, rewards may be viewed as incentives for executing actions. We will use $R_a(s_i,s_j)$ to represent $\mathcal{R}(s_i,a,s_j)$.
	%    \item an initial state $s_0\in \mathcal{S}$.
	
	%\item $\gamma \in [ 0,1 ] $ is the discount factor, which determines how far into the future satisfaction of requirements should affect computed strategies.
	
	% which reflects various degrees of preference to rewards earned sooner. %The discount factor gives present rewards are preferred over similar future rewards, and (2) convergence of the expectation of infinite reward series. This latter condition is necessary for the computation of MDP strategies since the utility function used for the evaluation of strategies is the {\it discounted expected linear additive} utility, i.e. $V^\pi(s)=u(R_t^{\pi_s}, R_{t+1}^{\pi_s},...)=\mathds{E}[ \sum_{t'=0}^{\infty} \gamma^{t'} R^{\pi_s}_{t+t'} ]$. .
\end{itemize}
Formally, a (memoryless) strategy is a mapping $\pi : \mathcal{S} \rightarrow \mathcal{A}$ from states to actions. An optimal strategy, denoted $\pi^*$, is the one which maximizes the {\it expected linear additive} utility, formally defined as $V^\pi(s)=%u(R_t^{\pi_s}, R_{t+1}^{\pi_s},...)=
\mathds{E}[ \sum_{t'=0}^{\infty} \gamma^{t'} R^{\pi_s}_{t+t'} ]$. %\bashar{maybe get rid of the equation}
Intuitively, this utility states that a strategy is as good as the amount of discounted reward it is expected to yield~\cite{Mausam2012}. Setting $\gamma=1$ expresses indifference of the agent to the time in which a particular reward arrives; setting it to a value $0\leq \gamma < 1$ reflects various degrees of preference to rewards earned sooner.\
%XXXNotice that in the context of this work, we set $0\leq \gamma=0.98 < 1$  to (1) ensure the convergence of the infinite reward series in the utility function definition; (2) give preference to the satisfaction of requirements that may be complied with in the near future over those which may only be complied with in a more distant future.

MDPs have a key property: solving an MDP finds an optimal strategy $\pi^*$, which is deterministic, Markovian and stationary. This means that computed strategies are independent of both past actions/states and time, which ensures their compactness and practicality. Furthermore, there exist practical algorithms for solving MDPs, e.g., value iteration and policy iteration. Both of these algorithms can be shown to perform in polynomial time for fixed $\gamma$~\cite{Littman}. %, but value iteration can take a number of iterations proportional to $1/(1-\gamma)log(1/(1-\gamma))$ in the worst case~\cite{littman1995complexity}. 
%Details and complexity of algorithms for solving MDPs can be found in \cite{Baier:2008:PMC:1373322,Mausam2012}.

 MDPs with memoryless strategies, depicted in Figure~\ref{fig:mdp_basic} (rounds are states and rounded squares are events), have however the following restrictions: 
%\begin{itemize}

	
	\paragraph*{The {\it implicit-event action model}~\cite{boutilier99}} MDPs do not support an explicit representation of exogenous events.  Figure~\ref{fig:mdp_events} shows exogenous events (in non-rounded squares connected with pointed line to states) that can occur with certain occurrence probabilities (in green in the figure) in every state. Exogenous events are an essential element to model aspects of the environment that are not controllable by the agent. They are the means to represent, for example, that customers can arrive at the restaurant or that they may request to order.
	
	\paragraph*{The Markovian assumption~\cite{Bacchus96,Bacchus97}} in MDP, reward and transition functions have to be Markovian, i.e., they can not refer to the history of previous states or transitions. Figure~\ref{fig:mdp_rewards} shows an example of a non-Markovian reward (described on the dashed transition), i.e., one that is entailed only if certain conditions are satisfied on the history of states and transitions. The support of non-Markovian rewards is necessary to associate transitions that satisfy requirements~\cite{Lamsweerde2009}, which are often conditional and can have deadlines, with rewards. %This is because typical software requirements~\cite{Lamsweerde2009} are often conditional and can have deadlines.
%\end{itemize}  


\begin{figure*}[!htb]
	%\resizebox{\textwidth}{0.1\textwidth}{
	\minipage{0.3\textwidth}
	\includegraphics[width=45mm, scale=0.45]{MDP_basic}
	\caption{Basic MDP model}\label{fig:mdp_basic}
	\endminipage\hfill
	\minipage{0.35\textwidth}
	\includegraphics[width=55mm, scale=0.5]{MDP_events}
	\caption{Support of Exogenous Events}\label{fig:mdp_events}
	\endminipage\hfill
	\minipage{0.3\textwidth}
	\includegraphics[width=50mm, scale=0.5]{MDP_rewards}
	\caption{Support of Non-Markovian Rewards}\label{fig:mdp_rewards}
	\endminipage
%}
\end{figure*}



%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth,height=0.5\linewidth]{illustrationLimitationsMDP3}
%	\caption[MDP Limitations]{MDP Model Limitations}
%	\label{fig:mdp_limitations}
%\end{figure}
%Figure~\ref{fig:mdp_limitations} illustrates MDP limitations. Figure~\ref{fig:mdp_limitations}(1) shows an MDP model with its states, actions, transitions and rewards. Figure~\ref{fig:mdp_limitations}(2) shows exogenous events that can occur with certain occurrence probabilities in every state. Exogenous events are an essential element to model aspects of the environment that are not controllable by the agent. They are the means to represent, for example, that customers can arrive at the restaurant or that they may request to order. 
%Figure~\ref{fig:mdp_limitations}(3) shows non-Markovian rewards, i.e. transition rewards that are dependent of the history of past states and transitions. Non-Markovian rewards are necessary to associate transitions that correspond to requirements satisfaction with rewards. This is needed since requirements~\cite{Lamsweerde2009} are often conditional and can be associated with deadlines. For example, a conditional achieve requirement may state that $RoboX$ must collect a customer's orders if the customer requests to order. In other words, the requirement is activated or becomes in force only after the customer requests to order. Similarly, requirements can have deadlines, e.g. if $RoboX$ has to collect the customer's order within at most 5 time units. The encoding of such requirements using Markovian rewards is not possible. Since general-purpose languages proposed by probabilistic model-checkers are intended to describe MDP models such the one shown in Figure~\ref{fig:mdp_limitations}(1), they do not support the description of exogenous nor of non-Markovian rewards shown in Figure~\ref{fig:mdp_limitations}(2) and (3). The following section discusses how our framework overcomes those limitations.

\subsection{Overview of the Construction of MDPs from \react Models}
\label{sec:mdp_construction}
The construction of MDPs based on \react models\footnote{The formal details can be found in \url{https://goo.gl/aoLh7i}.} relies on the following intuitions: %As just described, one may view an MDP as a LTS with probabilistic transitions which are associated with rewards representing the payoff/cost that are entailed when transitions are followed. %Formally, an MDP is a tuple $\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma \rangle$ and a domain model is a tuple $\langle \mathcal{SV}, \mathcal{AV}, \mathcal{EV}, \mathcal{RQ}, s_0 \rangle$ into an $MDP_r=\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma \rangle$. The translation of domain descriptions into MDP proceeds as follows:
\begin{itemize}
	\item the states and the (probabilistic) transitions of the LTS behind the MDP are constructed based on the variables, actions and events in the \react domain model;
	\item the rewards in the MDP are associated with transitions that lead to the satisfaction of requirements.%, since this is when there is a reward in the \react model.
\end{itemize}

\paragraph*{Dealing with the Markovian assumption} Building an MDP from an \react model requires the satisfaction of the Markovian assumption. In the context of this work, determining the satisfaction of requirements, with the exception of unconditional requirements, requires to keep track of history. To solve this issue, we extend the state space to store information that is relevant to determine the status of requirements in every state. This is done by associating every requirement with a state variable, whose value reflects the status of the requirement in the state\footnote{This technique is inspired by the state-based approach in~\cite{Bacchus96} to handle non-Markovian rewards, but is tailored to support requirements in \react.}. 
The value of those variables, called {\it requirements variables}, are updated whenever their corresponding requirement is activated, canceled, satisfied, etc.  

\textit{Requirements Variables $\mathcal{RV}$} are special variables whose domain represents all the possible statuses of their corresponding requirement. The statuses of requirements and their update after requirement activation, cancellation, satisfaction, etc are defined in the transitions part of Figures~\ref{fig:unconditionalRE} and \ref{fig:conditional_deadline}. On the other hand, the rewards part defines transitions that satisfy requirements and, consequently, entail a reward. 

For example, consider a conditional achieve requirement $CA$ of the form $\textbf{ReqID}\, m \,\textbf{achieve}\, S \,\textbf{if} \, A \,\textbf{unless} \, Z\,\textbf{reward} \, r$. This requirement is associated with a requirement variable $m$ whose domain includes the requirement's possible statutes $\{I,R\}$. %In the state $I$, the requirement is said to be {\it inactive}. In the state $R$, the requirement is said to be {\it in force}, i.e. it should be complied with. 
The transitions part of Figure~\ref{fig:conditional_deadline} shows the evolution of $CA$ requirements when their activation, cancellation and required conditions occur. It is to be read as follows: when the status is $I$ and the activation condition $A$ is true, then the status is updated to $R$. Analogously, if the status is $R$ and the cancellation condition $Z$ or the required condition $S$ is true, then the status is updated to $I$. %The update of the state of a requirement is performed by updating the value of the state variable that is associated with it. 
The updating of a state variable as just described enables the definition of a Markovian reward when requirements are satisfied. The rewards part of Figure~\ref{fig:conditional_deadline} shows transitions of $CA$ requirements that entail rewards. This figure should be read as follows: a requirement $m$ of type $CA$ induces a reward $r$ on a transition from a state $i$ to a state $j$ iff, in $i$, the required condition of $m$ does not hold and the status of $m$ is $R$; while $S$ holds in $j$.  


% The state machines of the different requirements and their associated transition rewards are shown in Figures~\ref{fig:unconditionalRE} and \ref{fig:conditional_deadline}. They comprise two parts: the transitions part describes every requirement’s state machine whereas the rewards part describes which transitions in the state machines entail rewards. More precisely, a reward is given on a transition whenever this transition satisfies the requirement. 

\paragraph*{Dealing with the absence of exogenous events} \react models have explicit-event models whereas MDPs impose an {\it implicit-event action} model. To overcome this limitation, we exploit the technique proposed in~\cite{boutilier99} which enables computation of {\it implicit-event} action transition matrices from explicit-event models. The use of this technique assumes the following rules: 1) the action in which exogenous events are folded, always occurs before it and 2) events are {\it commutative}, i.e., their order of occurrence from an initial state produces the same final state. Under those assumptions, which are satisfied in our running example, the {\it implicit-event} transition matrix $Pr_a(s_i,s_j)$ of an action $a$ is computed in two steps: first, the transition matrix of $a$ (without exogenous events) and the transition matrix and occurrence vector of every event $e$ are computed separately; then, those elements are used to construct the implicit-event matrix of every action $a$. This process is illustrated in the following section using an example. Note that it is possible to integrate other (more complex) interleaving semantics into the framework if necessary by changing the technique used to compute the {\it implicit-event} transition matrix~\cite{boutilier99}. %In the following, this process is illustrated through an example in the next section. 
%Interested readers are referred to~\cite{boutilier99} for further details.



%Note that the generalization of our approach to add support for Past Linear Temporal Logic as proposed in~\cite{Bacchus96} is left for future work. 

\subsection{MDP Construction Process}
An \react MDP $MDP_r=\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma \rangle$ is constructed from a model $\mathcal{D}_r=\langle \mathcal{SV}, \mathcal{AV}, \mathcal{ED}, \mathcal{RQ}, s_0 \rangle$ as follows. %For the sake of clarity, the construction of the MDP is presented the mapping informally here and present the formal description in Appendix~A. 
%Note that we do not consider the initial state $s_0$ in the discussion of the semantics: having an initial state only reduces the number of states when computing strategies to those that are {\it reachable} from the initial state. %Since it does not actually affect the semantics.
%The mapping can be summarized as follows.


\textit{States $\mathcal{S}$: }
represent all possible configurations of the system and the environment. A state is a specific {\it configuration}, i.e., an assignment of every state variable in $\mathcal{SV}$ and requirement variable in $\mathcal{RV}$ a value from their domain. %In order to enable the definition of Markovian reward functions, we further expand the state space such that every state include information about the state of every requirement $r\in \mathcal{R}$. 
%Thus, every state may be viewed as consisting of two parts: (1) a base state consisting of a specific configuration of state variables, and (2) an expanded state consisting of a specific configuration of requirements. %The state machines corresponding to the various requirement types are shown in Fig.~\ref{fig:statetransitionsrewards}.

For example, consider a domain model $\mathcal{D}_r$ comprising of two boolean variables $x$ and $y$ and one requirement $m$ of type $CA$. The set of states $\mathcal{S}$ constructed from $\mathcal{D}_r$ comprises all possible configurations of its state and requirement variables. Thus, $\mathcal{S}$ includes the eight states in Figure~\ref{fig:example-states}.

\begin{figure}[t]
	\centering
	\includegraphics[width=70mm, scale=0.7]{Example-States}
	\caption{Constructed States}
	\label{fig:example-states}
\end{figure}


\textit{Actions $\mathcal{A}$:} are all the actions appearing in $\mathcal{AV}$ of the domain model $\mathcal{D}_r$ extended with the empty action $noop$, which produces no effects and has no cost, i.e., $\mathcal{A}=\mathcal{AV}\cup\{noop\}$. %The empty action $noop$ is an action which produces no effects and has no cost.

\textit{The transition matrix $\mathcal{T}$:} is computed in two steps: first, the transition matrix of $a$ (without exogenous events) and the transition matrix and occurrence vector of every event $e$ are computed separately; then, those elements are used to construct the implicit-event matrix of every action $a$.
%To deal with the implicit-event model, we follow the technique proposed in~\cite{boutilier99} for computing an {\it implicit-event} transition matrix from an explicit-event model. %The use of this technique assumes the following rules: 1) the action in which the exogenous events is folded, always occurs before it and 2)  events are {\it commutative}, i.e. their order of occurrence from an initial state produces the same final state. %interleaving semantics for actions and events:
%\begin{itemize}
%	\item the action in which the exogenous events is folded, always occurs before it;
%	\item events are {\it commutative}, i.e. their order of occurrence from an initial state produces the same final state. %(a) for any initial state $s$ and any pair of events $e_1$ and $e_2$, the distribution that results from applying event sequence $e_1.e_2$ to $s$ is identical to that obtained from the sequence $e_2.e_1$; (b) the occurrence probabilities at intermediate states are identical. 
%\end{itemize}  
%\noindent %Under these conditions the combined transition distribution for any action a is computed by considering the probability of any subset of events and applying that subset in any order to the distribution associated with a?
%Under the previous assumptions, which are satisfied in our running example, the {\it implicit-event} transition matrix $Pr_a(s_i,s_j)$ of an action $a$ is computed in two steps: first, the transition matrix of $a$ (without exogenous events) and the transition matrix and occurrence vector of every event $e$ are computed separately; then, those elements are used to construct the implicit-event matrix of every action $a$ as proposed in~\cite{boutilier99}. In the following, we present the computation of explicit event and action matrices as well as of event occurrence vectors and illustrate the computation of {\it implicit-event} matrices through an example. Interested readers are referred to~\cite{boutilier99} for further details. 
%Specifying a transition function for an action and zero or more exogenous events is not generally easy for actions and events can interact in complex ways~\cite{boutilier99}. For example, true concurrency when, for example, if a robot lifts the side of atable on which a glass of water is situated, the water will; similarly if an exogenous event causes theother side to be raised. But if the action and event occur simultabeously, the result is different as the water is not spilled.  it is straightforward to consider other more 
%Under these conditions the com y bined transition distribution for an y action a is computed b y considering the probabilit y of an y subset of ev en ts and applying that subset in an y order to the distribution associated with a?
%\npaola{proposal for replacing the below sentence with this ``Note that the above assumptions imply that systems that do not guarantee them cannot benefit from \react as it is since the MDP construction is at the moment relies on them. However, there are different ways to overcome this limitation and we plan to explore them as future work. A possible option could be to integrate other (more complex) interleaving semantics into the framework and, if necessary, change the technique used to compute the {\it implicit-event} transition matrix. Another option could be to support exogenous events by constructing {\it action profiles} where each profile represents the concurrent execution of exactly one action and zero or more exogenous events. Finally, another way to model exogenous events could be through Markov games, where exogenous events can be seen as  the actions of another agent. The choice made in the current proposal was motivated by the simplicity of the computation and the semantics of MDPs of the former approach.'' }
 %There are also other ways to support exogenous events. For example, we could construct {\it action profiles} where each profile represents the concurrent execution of exactly one action and zero or more exogenous events. Markov games is another way to model exogenous events (as the actions of another agent). Our choice was motivated by the simplicity of the computation and the semantics of MDP of the former approach. %We intend to study Markov games in a future work.

%The transition matrix of $a$ (without event occurrences) is computed by identifying transitions that could result from executing $a$ in every state. The execution of $a$ in a state $s_i$ leads to another state $s_j$ with a probability $p$ iff: (1) the base state of $s_j$, denoted $\overline{s_j}$, is the result of executing one effect of the action $a$ in the base state of $s_i$, denoted $\overline{s_i}$, (2) the expanded state of $s_j$, denoted $\hat{s_j}$, satisfies the state transition models described in Figures~\ref{fig:unconditionalRE} and \ref{fig:conditional_deadline}, for every requirement $r\in \mathcal{R}$ in the expanded state of $s_i$, denoted $\hat{s_i}$, (3) $p$ is the probability of producing the effect.  

For example, consider that our domain model $\mathcal{D}_r$ includes one probabilistic action $a$, one deterministic action $b$ %\footnote{Notice that this definition of $b$ is similar to the definition of the $noop$ action.} 
and one requirement $m$, which are defined as follows:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\textbf{Action } a \textbf{ if } !x \textbf{ effects }  \langle x \textbf{ prob } 0.8 \rangle \langle y \textbf{ prob } 0.2 \rangle \; \textbf{ cost } 10\\ 
&\textbf{Action } b \textbf{ if } x \textbf{ effects }  \langle !x \rangle \; \textbf{ cost } 5\\ 
&\textbf{ReqID } m \textbf{ achieve } x \textbf{ if }  !x \textbf{ reward } 100
\end{align*} \endgroup

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Examples-Transitions}
	\caption{(1) action transitions, (2) implicit-event action transitions.}
	\label{fig:example-action-transition}
\end{figure}

\noindent Figure~\ref{fig:example-action-transition}(1) shows the transitions caused by the execution of actions in the states $s_2$ and $s_4$. For example, since the condition $!x$ is satisfied in $s_2$, the execution of $a$ in $s_2$ produces $x$ with a probability of $0.8$ and produces $y$ with a probability of $0.2$. Notice that after the execution of $a$, the base state of both $s_0$ and $s_4$ could be the result of executing action $a$ in $s_2$. However, since the execution of $a$ satisfies the requirement $m$, i.e., makes $x$ true, only the expanded state of $s_4$ satisfies the state transition model of the $CA$ requirement $m$ shown in Figure~\ref{fig:conditional_deadline} since $m=I$. Thus, the execution of $a$ in state $s_2$ leads to $s_0$ with a probability $0.8$, i.e., $Pr_a(s_2,s_4)=0.8$. The execution of $b$ and $noop$ do not change the state.%In particular, since the activation conditions 

% in the expanded state of $s_0$, the state of $r$ is $i$. Only the transition from state $s_2$ to state $s_4$ follow the state transition model in~Fig.\ref{fig:statetransitionsrewards} for requirements $\mathcal{R}$. More precisely, since the transition to 
%$s_4$ caused by the execution of $a$ in $s_2$ satisfies the activation condition of $m$ and since the state of $m$ in $s_2$ is $i$, then the state of $m$ in $s_4$ must be $r$. 

%according to the state transition model of a $CA$ requirement, there is a transition from state $i$ to a state $r$ if the condition $A$ is satisfied by the transition. In our example, the activation condition of $a$ is satisfied on the transition from $s_2$ to $s_4$ but not on the transition from $s_2$ to $s_0$\footnote{ Requirement conditions $X$ are satisfied on a transition from a state $s_i$ to a state $s_j$ after the execution of $a$ iff $s_j \cup \{a\} \models X$.}. The execution of $a$ in state $s_2$ leads to state $s_0$ with a probability $0.8$, i.e. $Pr_a(s_2,s_4)=0.8$.

Events are similar to actions with the exception that they have occurrence probabilities, do not have a cost and do not advance time since they occur {\it concurrently} with actions. Let $e$ be an event defined similarly to $a$ as follows:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\textbf{Event } e \textbf{ if } !x \textbf{ occur prob } 0.2 \textbf{ effects }  \langle x \textbf{ prob } 0.8 \rangle \langle y \textbf{ prob } 0.2 \rangle 
\end{align*} \endgroup
\noindent In this case, the transition matrix of $e$ is similar to that of $a$, i.e., $Pr_e=Pr_a$. The occurrence vector $O_e$ of $e$ represents the probability of occurrence of $e$ in every state. Since the condition $\neg x$ is satisfied in the states $s_2$, $s_3$, $s_6$ and $s_7$, $O_e(s_2)=O_e(s_3)=O_e(s_6)=O_e(s_7)=0.2$. %After the computation of the transition matrix of action $a$, the transition matrix of every event $e$ and its occurrence vector, the {\it implicit-event} matrix of every action is computed. 
Figure~\ref{fig:example-action-transition}(2) shows the {\it implicit-event} transitions for the states $s_2$ and $s_4$: in $s_2$, event $e$ may occur with a probability of $0.2$, thus its effects are {\it factored in} action transitions as shown in~Figure~\ref{fig:example-action-transition}(2); in $s_4$, the condition of $e$ is not satisfied and, therefore, it does not affect the computed transitions for the actions $noop$ and $a$. Due to the interleaving semantics where exogenous events (may) occur after action execution, the transition caused by $b$ in $s_4$ is affected due to the possibility that $e$ occurs after $b$. %Notice that even though the action $noop$ does not produce effects and $a$ is not executable in $s_4$, there are transitions from $s_4$ to $s_2$ due to the possibility of occurrence of the exogenous event $e$, as shown in~Figure~\ref{fig:example-action-transition}(2).  

\paragraph*{Construction of the reward matrix $\mathcal{R}$:} Transition rewards are affected by: (1) action costs and (2) satisfaction of requirements. In particular, a transition reward $R_a(s_i,s_j)$ is the sum of rewards obtained due to satisfaction of requirements on the transition from $s_i$ to $s_j$ minus the cost of $a$. For example, consider the transition from $s_2$ to $s_4$ caused by the execution of $a$ in $s_2$. On this transition, the  requirement $m$ is satisfied. Since the cost of executing $a$ is $10$, this transition will be associated with a reward of $100-10=90$, i.e., $R_a(s_2,s_4)=90$. %The same applies for the transition from $s_6$ to $s_0$.



\subsection{Requirements Transitions and Rewards}
This section explains the key intuitions behind the modeling of requirements in \react and their semantics.


\paragraph*{Unconditional Achieve and Maintain Rewards} A maintain requirement defines a condition that should be kept satisfied. Therefore, a reward is given to the agent whenever this condition holds over two consecutive states, see, e.g., $\br{UM}$ in Figure~\ref{fig:unconditionalRE}. On the other hand, an achieve requirement defines a condition that should be reached. Therefore, the agent is rewarded when this condition becomes true, i.e., when it does not hold in a state but holds in the next, e.g., see $\br{UA}$. %Fig.~\ref{fig:unconditionalRE} shows the state machines and reward conditions of unconditional requirements. 
\begin{figure}
	\centering
	\includegraphics[width=75mm, scale=0.75]{UnconditionalRequirements}
	\caption{Unconditional Requirements States and Rewards}
	\label{fig:unconditionalRE}
\end{figure}

\paragraph*{Conditional Requirements} The satisfaction of requirements is often necessary only after some condition $A$ becomes true, see for instance $\br{CA}$ and $\br{CM}$ in Figure~\ref{fig:conditional_deadline}. Those requirements are therefore modeled as state machines which are initially in an initial or inactive state $I$. When their activation condition $A$ occurs, a transition to a new state $R$ occurs. In a state $R$, the requirement is said to be {\it in force}, i.e., its satisfaction is required. While in $R$, the reward $r$ is obtained whenever the agent manages to comply with the required condition $S$. If the cancellation conditions $Z$ is detected while the requirement is in force, a transition to $I$ occurs, i.e., the requirement is canceled and has no longer to be fulfilled.
\begin{figure*}
	\centering
	\includegraphics[width=0.85\linewidth]{Conditional_Deadline}
	\caption{Conditional and Achieve Deadline Requirements States and Rewards}
	\label{fig:conditional_deadline}
\end{figure*}

%For example, consider a conditional achieve requirement $CA$ of the form $\textbf{ReqID}\; m \;\textbf{achieve}\; S \;\textbf{if} \; A \;$ $\textbf{unless} \; Z \; \textbf{reward} \; r$. This requirement is associated with a variable $m$ which domain includes the possible states of a conditional achieve requirement, namely the states $\{I,R\}$. %In the state $I$, the requirement is said to be {\it inactive}. In the state $R$, the requirement is said to be {\it in force}, i.e. it should be complied with. 
%The transitions part of Figure~\ref{fig:conditional_deadline} shows the evolution of the state machine of $CA$ requirements. It is to be read as follows: when the state of the requirement is $I$ and the activation condition $A$ is true, then the state of the requirement is updated to $R$. Analogously, when the state of the requirement is $R$ and the cancellation condition $Z$ or the required condition $S$ is true, then the state of the requirement is updated to $I$. The update of the state of a requirement is performed by updating the value of the state variable that is associated with it. The updating of a state variable as just described enables the definition of a Markovian reward when the requirement is satisfied. The association of the satisfaction of a $CA$ requirement with a reward is depicted in the rewards part of Figure~\ref{fig:conditional_deadline}. This figure should be read as follows: the requirement $m$ induces a reward $r$ on the transition from some state $i$ to a state $j$ if the requirement's state in $i$ is $R$, and the required condition $S$ holds in $j$ and does not hold in $i$.  
%Fig.~\ref{fig:conditional_deadline} shows the textual representation, state machines and reward conditions of conditional requirements. 


\paragraph*{Deadline Achieve Requirements} Requirements are sometimes associated with fixed deadlines. Fixed deadlines can represent either an exact time after which the agent should comply with the requirement, see for example $\br{DEA}$ in Figure~\ref{fig:conditional_deadline}; or a period of (discrete) time during which the agent may comply at any moment, see for example $\br{DFA}$. In both cases, deadlines are modeled similarly. For example, consider a requirement $m$ having a deadline $D$. After $m$'s activation, a transition to a state $A(D)$ occurs. At every subsequent time unit, a transition from a state $A(X)$ to a state $A(X-1)$ occurs (unless $X=1$). A transition entails the requirement's reward if the requirement is satisfied on this transition. 




\comments{
	\begin{figure}
		\centering
		\includegraphics[width=\linewidth]{DeadlineAchieveRequirements}
		\caption{Deadline Achieve Requirements: State Machines and Associated Rewards}
		\label{fig:deadlineARE}
	\end{figure}
}

==> Submission Arxiv/Syntax.tex <==
%\subsection{Model Elements}
%\label{sec:syntax}
%Elements of a \react model define the system, its environment, its capabilities (its actions), exogenous events which may occur and the system requirements. 
The computation of {\it optimal strategies} is based on a {\it domain model}. A domain model specifies the environment, the capabilities of the autonomous system (or agent) and its requirements. Formally, an \react model ($\mathcal{D}_r$) is a tuple $\langle \mathcal{SV}, \mathcal{AD}, \mathcal{ED}, \mathcal{RQ}, s_c \rangle$ where: 
\begin{itemize}
	\item $\mathcal{SV}$ is a finite set of state variables with finite domains. State variables describe the possible states, i.e., the configuration of the software system and the environment;
	\item $\mathcal{AD}$ is a finite set of action descriptions representing the means that are available to the agent to change the system state, i.e. update the state variables $\mathcal{SV}$;
	\item $\mathcal{ED}$ is a finite set of event descriptions to represent the uncontrollable occurrences in the environment, i.e., events that change the state beyond the agent's control.
	\item $\mathcal{RQ}$ is a finite set of requirements, i.e., the (operationalisable) goals that the software system should satisfy;
	\item $s_c$ is the initial state of the system %(which can not be specified), 
	determined by the agent's monitoring components and sensors.
\end{itemize}
 An \react model has a corresponding textual representation called its {\it domain description}. It is formalized in the following using a variant of Backus-Naur Form (BNF): the names enclosed in angular brackets identify non-terminals, names in bold or enclosed within quotation marks are terminals, optional items are enclosed in square brackets,~$|$ is "or", items repeated one or more times are suffixed with $+$ and parentheses are used to group items together.%\bashar{Refer to a tech report for full spec of the language} 

\subsection{State, Actions and Events} 
\paragraph*{State Variables ($\mathcal{SV}$)} define the possible {\it states}, i.e., configurations of the software system and the environment. A variable $x\in \mathcal{X}_s$ is a multi-valued variable with a corresponding domain, denoted $dom(x)$. Every value $y\in dom(x)$ is a configuration of $x$. A state variable is defined as follows:
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\br{SV} ::= \textbf{Variable}\textbf{ } \br{ID} \, \textbf{domain} \,  ``\{" \, \br{VALS} \, ``\}"\\
&\br{VALS} ::= \br{ID} \, | \, \br{ID} \, ``," \, \br{VALS}  
\end{align*} \endgroup

\noindent where $\br{ID}$ is {\it text}, i.e., a concatenation of letters, digits and symbols. For example, we can represent the location of $RoboX$ and the status of tables at the restaurant using the following variables:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}%
\begin{align*}
&\textbf{Variable } location \textbf{ domain } \{atTable_1,atTable_2,atTable_3,\\
& \hspace{0.5cm}\hspace{0.5cm} atTable_4,inDining\_room,inKitchen,inOffice\}\\
&\textbf{Variable } table_i \hspace{1cm}(\forall \, 1\leq i \leq 4)\\
& \hspace{0.5cm}\textbf{ domain } \{empty,occupied,requested,received,\\
& \hspace{0.5cm}\hspace{0.5cm}in\_preparation,ready,collected,delivered,paid\}
\end{align*}
\endgroup
\noindent The variable $location$ defines the possible locations of $RoboX$. The variables $table_i$ represent the status of tables: when there are no customers at $table_i$, then $table_i\text{=}empty$. When a customer arrives and sits at the table, $table_i$ becomes $occupied$. Figure~\ref{fig:tablelts} depicts the update of the value of $table_i$ with the occurrence of the robot actions \{{\it get\_order, give\_order, collect\_order, deliver\_ order, clean\_table}\} and the exogenous events \{{\it customer\_arrives, customer\_orders, kitchen\_notification, custo\-mer\_pays}\}. In contrast to actions, exogenous events have an occurrence probability denoting their likelihood in a given situation. Actions, on the other hand, have a cost that represent the effort or price of their execution. Both exogenous events and actions do not have to be deterministic, i.e., their execution can have various effects, each with a different probability (in pink in the figure). 


\comments{When $RoboX$ asks the customer to order, $table_i\text{=}requested$. When the customer places an order, $table_i\text{=}order\_received$. After $RoboX$ gives the order to the kitchen, $table_i\text{=}in\_preparation$. After the kitchen notifies $RoboX$ that food is ready, $table_i\text{=}ready$. When $RoboX$ collects the food from the kitchen, $table_i\text{=}collected$. After food is delivered to the table, $table_i\text{=}delivered$. After the customer pays the bill and leaves, $table_i\text{=}paid$. When $RoboX$ cleans the table, $table_i\text{=}empty$.
}
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{TableStatus}
	\caption{A simplified model of serving a table at restaurant $FoodX$.}
	\label{fig:tablelts}
\end{figure*}
Variables which are not explicitly defined are considered to be boolean, i.e., their domain is $\{tt,\textit{ff}\}$. The notations $id$ and $!id$ are used as shortcuts for $id\text{=}tt$ and $id\text{=}\textsl{ff}$, respectively. %In this case, their domain does not have to be declared as they are assigned the domain $\{tt,ff\}$. Furthermore, for an $id\in \br{ID}$, the notations $id$ and $!id$ are used as a shortcuts for $id\text{=}tt$ and $id\text{=}ff$ respectively. 
The following declaration defines a boolean variable to represent that customers sitting at a table had looked at the menu.
%\npaola{What is the point of the example below ($looking_i$)?? Not clear what it is and why it is there!}
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\textbf{Variable } looked_i &(\forall \, 1\leq i \leq 4)
\end{align*}
\endgroup

\paragraph*{Actions ($\mathcal{AD}$)} are means that are available to the agent to change the system state. An action description is an expression $\br{AD}$ that is defined as follows:
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\br{AD} ::= \textbf{Action} \, \br{ID} \, \br{PEFFS}^+ \, [\textbf{cost} \, \br{\mathds{N}}]\\
&\br{PEFFS} ::= \textbf{ if } \br{CND} \textbf{ effects }  \br{EFFS}^+ \\
&\br{EFFS} ::= ``\langle" \br{EFF}^+ \,[ \textbf{prob } \br{P}] ``\rangle"\\
&\br{CND} ::= \br{ATOM} \,| \, \br{BL} \,| \,``!" \br{CND}\, | \,\br{CND} \\
& \hspace{0.5cm}  \, ``{\bf \&}" \, \br{CND} \,| \, \br{CND} \, ``{\bf ||}" \, \br{CND}  \,| \, ``(" \br{CND} ``)"\nonumber\\
&\br{EFF} ::=  \br{ID} ``{\bf =}" \br{ID}\\
%\br{ATOM} ::= \br{ID_a} \, |\, \br{ID_e} \, |\,\br{ID_s} \, | \, !\br{ID_s} \,| \, \br{ID_s} {\bf =} \br{ID_v}\\
&\br{ATOM} ::= \br{ID} \, | \, ``!"\br{ID} \,| \, \br{ID} ``{\bf =}" \br{ID}\\
&\br{BL} ::= ``true" \, | \, ``false"
\end{align*} \endgroup

%\npaola{Since the = in EFF has two different meaning (roughly speaking, assignment vs comparison) shouldn't be use two different symbols (= vs ==)? If so, examples need to be changed accordingly.}
\noindent %where $P$ is a number between zero and one. 
Actions can have a cost representing the difficulty level or effort necessary to execute it. Action costs are useful to trade-off the satisfaction of requirements with the required effort and, when not specified, are set to zero. 
In the following example, the cost of moving to $table_i$ is set to $10$.
\comments{
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}% \begin{align*}
&\textbf{Action } move\_to\_table_i&(\forall \, 1\leq i \leq 4)\\
& \hspace{1cm} \textbf{ if } location=inDining\_room \textbf{ effects }\langle location=atTable_i \rangle \\
& \hspace{1cm}\textbf{ cost } 10
\end{align*}
\endgroup
While in the above example the effect associated to the action is only one and so it will happen with probability $1$, in general
the effect of an action is probabilistic, i.e., different effects correspond to an action and each effect is associated with a certain probability to occur,
%On the other hand, effects of an action can be associated with a probability denoting the likelihood that the action execution produces them. 
For example, it is possible to specify that the action to move to the kitchen from the dining room has the desired effect with probability and does not bring any change with probability $20\%$: 
}
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\textbf{Action } move\_to\_kitchen \textbf{ if } location\text{=}inDining\_room\\
&\hspace{0.5cm} \textbf{ effects } \langle location\text{=}inKitchen \textbf{ prob } 0.8 \rangle\\
&\hspace{1cm} \langle location\text{=}inDining\_room \textbf{ prob } 0.2 \rangle \hspace{0.5cm} \textbf{ cost } 10
\end{align*}
\endgroup


Note that an expression $\br{AD}$ is well-formed only if (1) its various $\br{CND}$ are disjoint, i.e., they cannot be satisfied at the same time and (2) for every $\br{PEFFS}$, the sum of the probabilities $\br{P}$ of its subexpressions $\br{EFFS}$ is one, i.e., $\sum_{i=1}^{|\br{EFFS}|}\br{P}=1$. Note that we allow $\sum_{i=1}^{|\br{EFFS}|}\br{P}$ to be less than one. In this case, action execution has no effect with a probability of $1-\sum_{i=1}^{|\br{EFFS}|}\br{P}$. For example, this makes it possible to remove the second effect, $\langle location=inDining\_room \textbf{ prob } 0.2 \rangle$, from the previous action description without affecting the action semantics.

%\npaola{Which is the meaning go using angular brackets in the example(s)? They are not part of the grammar! Used all over the paper.}
%Notice that it is also possible to model actions with only an effect which will happen with probability $1$. For example, it is possible to state that the action to move to a table has a cost of 10 and that it succeeds with a probability of 80\% as follows.  
%For example, it is possible to specify that $RoboX$ can move to $table_i$ if it is in the dining room as follows:
%\begingroup\makeatletter\def\f@size{9}\check@mathfonts
%\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}% \begin{align*}
%&\textbf{Action } move\_to\_table_i\hspace{1cm}(\forall \, 1\leq i \leq 4)\\
%& \hspace{1cm} \textbf{ if } location=inDining\_room \textbf{ effects } \langle location=atTable_i \rangle
%\end{align*}
%\endgroup
%}

\paragraph*{Events ($\mathcal{EV}$)} represent occurrences that are not controlled by the agent. They may happen in the environment at any moment. An event description is expressed as follows:
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&\br{EV} ::= \textbf{Event} \, \br{ID} \, \br{PEFFS}^+ \\
&\br{PEFFS} ::= \textbf{ if } \br{CND} \, [\textbf{occur prob}\, \br{P} ]  \, \textbf{ effects } \br{EFFS}^+ 
\end{align*} 
\endgroup

\comments{
For example, it is possible to model the effects of a customer request to order using an {\it exogenous} event description as follows:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}% \begin{align*}
&		\textbf{Event } request\_to\_order_i\hspace{1cm}(\forall \, 1\leq i \leq 4)\\
& \hspace{1cm} \textbf{ if } table_i=occupied \textbf{ effects } table_i=requested
\end{align*}
\endgroup
}
Events are conditional and can occur with a different probability depending on the situation. %By default, it is assumed that the occurrence probability of exogenous events is zero. 
For instance, we can represent that customers may order with a higher probability if they had looked at the menu as follows:
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&		\textbf{Event } request\_to\_order_i \hspace{1cm}(\forall \, 1\leq i \leq 4)\\
& \hspace{0.5cm}\textbf{ if } table_i\text{=}occupied \,\&\, looked_i \textbf{ occur prob } 0.9\\
&\hspace{1cm} \textbf{ effects } \langle table_i\text{=}requested \rangle\\
& \hspace{0.5cm}\textbf{ if } table_i\text{=}occupied\, \& \, !looked_i \textbf{ occur prob } 0.2\\
&\hspace{1cm} \textbf{ effects } \langle table_i\text{=}requested \rangle
\end{align*}
\endgroup
\subsection{Requirements}
\label{sec:modeling_requirements} Requirements represent the objectives of the autonomous system. Every requirement is associated with a reward denoting its importance. %If a reward is not specified, the requirement is considered to have an arbitrary positive reward value of 1000. 
\react currently supports fourteen requirement types, which build upon and extend the goal patterns of the KAOS goal taxonomy~\cite{Letier2002}. Requirements are expressions:
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&		\br{RE} ::= \textbf{ ReqID } \br{ID} \, \br{REP}\\
& \br{REP} ::= ((\br{UA} \, | \, \br{UM} \,| \, \br{CA} \, | \, \br{DEA} \, | \, \br{DFA} \, | \, \br{CM} \, |  \\
&\hspace{0.5cm}\, \br{DEM} \, | \, \br{DFM}  \, \br{PM} \, | \, \br{PDEM} \, | \,  \br{PDFM}) \,[\textbf{reward } \mathds{N}]) \,|\, \nonumber\\
& \hspace{0.5cm} ((\br{RPM} \, | \, \br{RPDEM} \, | \, \br{RPDFM}) \,[\textbf{reward\_once } \mathds{N}])\nonumber
\end{align*} \endgroup
\noindent A requirement's type is determined based on whether it: is conditional (C) or unconditional (U); is a {\it maintain} (M) or {\it achieve} (A) requirement: duration of {\it maintain} requirements can be time-limited and its compliance can be best-effort (P) or strict (PR), i.e., during its duration the requirement does not have to be ``always'' satisfied; has a deadline (D), which can be exact (E), i.e., the requirement has to be satisfied at the deadline, or flexible (F), the requirement has to be satisfied within the deadline.
\comments{
\noindent A requirement's type is determined based on whether it:
\begin{itemize}
	\item is conditional (C) or unconditional (U);
	\item is a {\it maintain} (M) or {\it achieve} (A) requirement: duration of {\it maintain} requirements can be time-limited and its compliance can be best-effort (P) or strict (RP), i.e., during its duration the requirement does not have to be ``always'' satisfied;
	\item has a deadline (D), which can be exact (E) or flexible (F), i.e., the requirement has to be satisfied at or within the deadline respectively.
\end{itemize}
}
Due to space limitations, we only present unconditional, conditional and achieve deadline requirements. %For further details, please refer to~\cite{tech_report}.%Note also that it is straightforward to add support of new requirement types. % The syntax of the other requirements is shown in Fig.~(\ref{fig:unconditionalRE})(\ref{fig:conditionalRE})(\ref{fig:deadlineRE})(\ref{fig:durationRE}) and explained using examples in the next section. 

%\paola{May be you can at least say what the acronyms stand for. Moreover, are rewards associated only to two types of requirements? Why?}
%\comments{
% \begingroup\makeatletter\def\f@size{9}\check@mathfonts
%\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
%\begin{align*}
%&  \br{UA} ::= \textbf{achieve} \, \br{CND}\nonumber\\
%%& \br{UM} ::= \textbf{maintain} \, \br{CND}\nonumber\\
%& \br{CA} ::= \textbf{achieve} \, \br{CND} \, \textbf{if} \,\br{CND} \,[\textbf{unless} \, \br{CND}] \nonumber\\
%&  \br{UM} ::= \textbf{maintain} \, \br{CND}\nonumber\\
%%& \br{UM} ::= \textbf{maintain} \, \br{CND}\nonumber\\
%& \br{CM} ::= \textbf{maintain} \, \br{CND} \, \textbf{if} \,\br{CND} \,[\textbf{unless} \, \br{CND}] \nonumber
%%&  \br{DEA} ::=  \textbf{achieve} \, \br{CND} \, \textbf{within} \, \mathds{N}\, \textbf{if} \,\br{CND} %\,[\textbf{unless} \, \br{CND}]\nonumber\\
%%&  \br{DFA} ::=  \textbf{achieve} \, \br{CND} \, \textbf{after} \, \mathds{N}\, \textbf{if} \,\br{CND} %\,[\textbf{unless} \, \br{CND}]\nonumber\\
%%&  \br{PDEM} ::=  \textbf{maintain} \, \br{CND} \, \textbf{for} \, \mathds{N}\,  \textbf{after} \, %\mathds{N}\,\textbf{if} \,\br{CND} \,[\textbf{unless} \, \br{CND}]\nonumber\\
%%&  \br{PDFM} ::=  \textbf{maintain} \, \br{CND} \, \textbf{for} \, \mathds{N}\,  \textbf{within} \, %\mathds{N}\,\textbf{if} \,\br{CND} \,[\textbf{unless} \, \br{CND}]\nonumber
%\end{align*} \endgroup
%%\begin{figure}[t]
%%	\centering
%%	\includegraphics[width=0.7\linewidth]{IdentifyingRequirementType}
%%	\caption{Identification of Requirement Types}
%%	\label{fig:identifyingrequirementtype}
%%\end{f}
%}

\comments{
\noindent\paragraph*{On Rewards for Maintain Requirements with Duration} In addition to prioritization of requirements, rewards play a second role in the case of maintain requirements which have a fixed duration. In particular, rewards can be given either
\begin{itemize}
	\item at every time step the requirement is complied with,
	\item only if the requirement is complied with throughout its whole duration.
\end{itemize}
\noindent In the former case, {\it partial-compliance} is rewarded, i.e., the agent could envisage to violate the requirement for a period of time if the satisfaction of other requirements is more important and then go back to comply with the requirement again. In the latter case, the agent would have to choose between either {\it full-compliance} or {\it non-compliance} since {\it partial-compliance} is not rewarded. 
}


\textit{Unconditional Requirements:} denote conditions that have to be always maintained or (repeatedly) achieved. 
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&  \br{UA} ::= \textbf{achieve} \, \br{CND} && \br{UM} ::= \textbf{maintain} \, \br{CND}
\end{align*} \endgroup


\noindent For example, a $\br{UM}$ requirement to remain in the dining room or an $\br{UA}$ to ensure that $table_1$ repeatedly pays.
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&	 \textbf{ReqID } req_1 \textbf{ maintain } location\text{=}inDining\_room \nonumber\\
&	 \textbf{ReqID } req_2 \textbf{ achieve } table_1\text{=}paid \nonumber
\end{align*} \endgroup
%\noindent which are satisfied when the $location$ is always the dining room and when the status of $table_1$ is repeatedly paid, respectively.
%\noindent The main difference between an unconditional maintain ($UM$) and an unconditional achieve ($UA$) is that the reward associated to $UA$ is obtained only when the required condition is {\it achieved} for the first time. 

\textit{Conditional Requirements:} should be satisfied only after some given conditions are true. They can have a cancellation condition after which their satisfaction is no longer required. 
 \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
& \br{CA} ::\text{=} \textbf{achieve} \, \br{CND} \, \textbf{if} \,\br{CND} \,[\textbf{unless} \, \br{CND}] \\
& \br{CM} ::\text{=} \textbf{maintain} \br{CND} \textbf{if} \br{CND} \,[\textbf{unless} \, \br{CND}] 
\end{align*} \endgroup
\noindent For example, $RoboX$ may have to get the order from $table_i$ only if $table_i$ requests to order, or it should remain in the dining room after it gets $table_1$ until $table_1$'s order is served.
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&		\textbf{ReqID } req_3 \textbf{ achieve } table_i\text{=}received\\
& \hspace{0.5cm} \textbf{ if } table_1=requested \textbf{ reward } 100\\
&		\textbf{ReqID } req_4 \textbf{ maintain } location=inDining\_room \\
& \hspace{0.1cm}\textbf{ if } table_1\text{=}requested \textbf{ unless } table_1\text{=}received \textbf{ reward } 100
\end{align*}
\endgroup

\textit{Deadline Requirements:} must be satisfied after an exact number of time instants or within a period of time:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
& \br{DEA} ::= \textbf{achieve} \, \br{CND} \,  \textbf{after} \,\mathds{N}_{+} \, \textbf{if} \,\br{CND} \,[\textbf{unless}  \,\br{CND}] \\
& \br{DFA} ::= \textbf{achieve} \, \br{CND} \,  \textbf{within} \,\mathds{N}_{+} \, \textbf{if} \,\br{CND} \,[\textbf{unless} \,\br{CND} ] 
\end{align*}
\endgroup

For example, $RoboX$ may have to be at $table_1$ within at most 4 time units after $table_1$ requests to place an order, or it may have to be at the kitchen after exactly 4 time units after it receives a notification that food is ready.
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}} 
\begin{align*}
&		\textbf{ReqID } req_5 \textbf{ achieve } location\text{=}atTable_1 \textbf{ within } 4\\
& \hspace{0.5cm} \textbf{ if } table_1\text{=}requested \textbf{ reward } 100\\
&		\textbf{ReqID } req_6 \textbf{ achieve } location\text{=}inKitchen \textbf{ after } 4\\
& \hspace{0.5cm} \textbf{ if } table_1\text{=}ready  \textbf{ reward } 100
\end{align*}
\endgroup

\noindent In the following, we use the terms {\it name}, {\it required condition}, {\it activation condition}, {\it cancellation condition} and {\it deadline} to refer to the parts of a requirement expression that come after $`\text{ReqID'}$, $`\text{achieve'}$ or $`\text{maintain'}$, $`\text{if'}$, $`\text{unless'}$ and $`\text{after'}$ or $`\text{within'}$ parts of the requirement expression respectively. %For example, consider the requirement $req_4$. The requirement's name is $req_4$, its required condition is $location=charging\_station$, its activation and cancellation conditions are $battery=empty$ and $!battery=empty$ respectively.


